Interference Channels with Rate-Limited Feedback

We consider the two-user interference channel with rate-limited feedback. Related prior works focus on the case where feedback links have infinite capacity, while no research has been done for the rate-limited feedback problem. Several new challenges arise due to the capacity limitations of the feedback links, both in deriving inner-bounds and outer-bounds. We study this problem under three different interference models: the El Gamal-Costa deterministic model, the linear deterministic model, and the Gaussian model. For the first two models, we develop an achievable scheme that employs three techniques: Han-Kobayashi message splitting, quantize-and-binning, and decode-and-forward. We also derive new outer-bounds for all three models and we show the optimality of our scheme under the linear deterministic model. In the Gaussian case, we propose a transmission strategy that incorporates lattice codes, inspired by the ideas developed in the first two models. For symmetric channel gains, we prove that the gap between the achievable sum-rate of the proposed scheme and our new outer-bounds is bounded by a constant number of bits, independent of the channel gains.

==> DICachievableregion.tex <==
We provide the outline of our achievable scheme. We employ block Markov encoding with a total size $B$ of blocks. In block 1, each transmitter splits its own message into common and private parts and then sends a codeword superimposing the common and private messages. For power splitting, we adapt the idea of the simplified Han-Kobayashi scheme~\cite{dtse:it07} where private power is set such that a private signal is seen below the noise level at the other receiver. In block 2, with feedback, each transmitter decodes the other user's common message (sent in block 1) while treating the other user's private signal as noise. Two common messages are then available at the transmitter: (1) its own message; and (2) the other user's message decoded with the help of feedback. Conditioned on these two common messages, each transmitter generates new common and private messages. It then sends the corresponding codeword. Each transmitter repeats this procedure until block $B-1$. In the last block $B$, to facilitate backward decoding, each transmitter sends the predetermined common message and a new private message. Each receiver waits until total $B$ blocks have been received and then performs backward decoding.


\subsection{Codebook Generation}

Fix a joint distribution $p(u)p(u_1|u) p(u_2|u) p(x_1|u_1, u)p(x_2|u_2,u)$.
%Based on $p(u)$, we first generate a codeword $u^{N}$ where $N$ is the codeword length.
%The issue is how to generate $v_1^N$ and $v_2^N$. Since the given distribution does not include $v_1$ and $v_2$, it seems impossible to generate them. However, explicit functional relationship between $x_1$ and $v_1$ makes it possible.
Write a joint distribution $p(u,u_1,u_2, v_1, v_2, x_1,x_2)$ in two different ways:
\begin{align}
\begin{split}
&p(u,u_1, u_2, v_1,v_2,x_1,x_2) \\
&= p(u)p(u_1|u)p(u_2|u) p(x_1|u, u_1)p(x_2|u, u_2) \delta (v_1 - g_1(x_1))  \delta (v_2-g_2(x_2)) \\
&= p(u)p(u_1|u)p(u_2|u) p(v_1|u, u_1)p(v_2|u,u_2) p(x_1|u,u_1,v_1) p(x_2|u, u_2, v_2)
\end{split}
\end{align}
where $\delta(\cdot)$ indicates the Kronecker delta function. From this, we get
\begin{align}
\begin{split}
p(x_1|u, u_1, v_1) := \frac{p(x_1|u, u_1) \delta(v_1 - g_1(x_1))}{p(v_1|u, u_1)} \\
p(x_2|u, u_2, v_2) := \frac{p(x_2|u, u_2) \delta(v_2 - g_2(x_1))}{p(v_2|u, u_2)}.
\end{split}
\end{align}

First transmitter 1 generates $2^{N(R_{1cc} +R_{2cc}) }$ independent codewords $u^N(i,j)$ according to $\prod_{i=1}^{N} p(u_i)$, where $i \in \{1, \cdots, 2^{NR_{1cc}} \}$ and $j\in \{1, \cdots, 2^{NR_{2cc}} \}$. For each codeword $u^N(i,j)$, it generates $2^{NR_{1cc}}$ independent codewords $u_1^{N}((i,j),k)$ according to $\prod_{i=1}^{N} p(u_{1i}|u_i)$ where $k \in \{1, \cdots, 2^{NR_{1cc}} \}$. Subsequently, for each pair of codewords $\left( u^N(i,j),u_1^N((i,j),k) \right) $, generate $2^{NR_{1nc}}$ independent codewords $v_1^N((i,j),k,l)$ according to $\prod_{i=1}^{N} p(v_{1i}|u_i, u_{1i})$ where $l \in \{1, \cdots, 2^{NR_{1nc}} \}$. Lastly, for each triple of codewords  $\left( u^N(i,j),u_1^N((i,j),k),v_1^N((i,j),k,l) \right) $, generate $2^{NR_{1p}}$ independent codewords $x_1^N((i,j),k,l,m)$ according to $\prod_{i=1}^{N} p(x_{1i}|u_i, u_{1i}, v_{1i})$ where $m \in \{1, \cdots, 2^{NR_{1p}} \}$.
Similarly, transmitter 2 generates codewords $u_2^N$, $v_2^N$ and $x_2^N$.

On the other hand, receiver 1 generates $2^{N \hat{R}_1}$ sequences $\hat{y}_1^N (q)$ according to $\prod_{i=1}^{N} p(\hat{y}_{1i})$ where $q \in \{1, \cdots, 2^{N\hat{R}_{1}} \}$. Similarly, receiver 2 generates $\hat{y}_2^N$.

\textit{Notation:} Notations are independently used only for this section. The index $k$ indicates the cooperative common message of user 1 instead of user index. The index $i$ is used for both purposes: (1) indicating the previous common message of user 1; (2) indicating time index. It could be easily differentiated from contexts.

\subsection{Feedback Strategy}
We employ block Markov encoding with a total size $B$ of blocks. Focus on the $b$th block transmission. Given the received signal $y_1^{N,(b)}$ for block $b$, receiver 1 finds an index $q$ such that
$\left( \hat{y}_1^{N,(b)}(q), y_{1}^{N,(b)} \right) \in \mathcal{T}_{\epsilon}^{N}$.
Then, by the covering lemma in~\cite{ElGamalKim:NIT}, the probability that there is no such an index becomes arbitrarily small (as $N$ goes to infinity) if
\begin{align}
\label{eq:tildeR1}
\hat{R}_1 \geq I(\hat{Y}_1; Y_1).
\end{align}
Now partition the set of indices $q\in [1:2^{N \hat{R}_1}]$ into equal-size subsets (bins)
\begin{align*}
\mathcal{B}(r)=\left[ (r-1) 2^{N(\hat{R}_{1}- C_{\sf FB1}) }+1: r 2^{N(\hat{R}_{1}- C_{\sf FB1}) } \right],\; r \in [1:2^{N C_{\sf FB1}}].
\end{align*}
Receiver 1 then feeds back the bin index $r$ such that $q \in \mathcal{B}(r)$.
Using $r$, transmitter 1 finds an unique index $q \in \mathcal{B}(r)$ such that
$\left( \hat{y}_1^{N,(b)}(q), x_{1}^{N,(b)}, u^{N, (b)} \right) \in \mathcal{T}_{\epsilon}^{N}$. By packing lemma~\cite{ElGamalKim:NIT}, the decoding error probability goes to zero if
\begin{align}
\label{eq:constraintY1tilde}
\hat{R}_1 - C_{\sf FB1} \leq I(\hat{Y}_1; X_1, U).
\end{align}
Using~(\ref{eq:tildeR1}) and~(\ref{eq:constraintY1tilde}), we get
\begin{align}
\label{eq:constraint2Y1tilde}
I(\hat{Y}_1; Y_1 |X_1, U ) \leq C_{\sf FB1},
\end{align}
Similarly, for a communication pair of transmitter 2 and receiver 2, we get
\begin{align}
\label{eq:constraint2Y2tilde}
I(\hat{Y}_2; Y_2 |X_2, U ) \leq C_{\sf FB2}.
\end{align}

\subsection{Encoding}
Given $\hat{y}_1^{N,(b-1)}$ (decoded with the help of feedback), transmitter 1 finds an unique index $\hat{w}_{2cc}^{(b-1)} = \hat{k}$ (sent from transmitter 2 in the $(b-1)$th block) such that
\begin{align*}
\begin{split}
&\left( u^N \left( \cdot \right), u_1^N \left( \cdot \right), v_1^N (\cdot), x_1^N (\cdot), u_2^N ( \cdot, \hat{k} ) , y_1^{N,(b-1)}  \right) \in \mathcal{T}_{\epsilon}^{(N)},
\end{split}
\end{align*}
where $(\cdot)$ indicates the known messages $(w_{1cc}^{(b-2)}, \hat{w}_{2cc}^{(b-2)}, w_{1nc}^{(b-1)}, w_{1p}^{(b-1)})$. We assume that $\hat{w}_{2cc}^{(b-2)}$ is correctly decoded from the previous block $(b-1)$. By the packing lemma~\cite{ElGamalKim:NIT}, the decoding error probability becomes arbitrarily small (as $N$ goes to infinity) if
\begin{align}
\begin{split}
\label{eq-R2c-constraint}
R_{2cc} &\leq I(U_2;\hat{Y}_1|X_1,U) = I(\hat{Y}_1; Y_1|U, X_1) - I(\hat{Y}_1;Y_1|U, U_2, X_1)\\
&\leq  \min ( C_{\sf FB1} - \delta_1, I(U_2;Y_1|X_1,U)  ),
\end{split}
\end{align}
where the second equality follows from~(\ref{eq:constraint2Y1tilde}) and the third inequality is due to the fact that $\delta_1:= I(\hat{Y}_1; Y_1| U, U_2, X_1)$ and $I(U_2;\hat{Y}_1|X_1,U) \leq I(U_2;Y_1|X_1,U)$.
%Note that
%\begin{align*}
%I(U_2;\hat{Y}_1|X_1,U) &\leq I(V_2,U_2;\hat{Y}_1,Y_1|X_1,U) = I(V_2;\hat{Y}_1,Y_1|X_1,U) + I(U_2; \hat{Y}_1,Y_1|X_1,U,V_2) \\
%&= I(V_2;Y_1|X_1,U) + I(V_2;\hat{Y}_1|X_1,U,Y_1) = I(V_2;Y_1|X_1,U).
%\end{align*}

Based on $(w_{1cc}^{(b-1)},\hat{w}_{2cc}^{(b-1)})$, transmitter 1 generates a new cooperative-common message $w_{1cc}^{(b)}$, a non-cooperative-common message $w_{1nc}^{(b)}$ and a private message $w_{1p}^{(b)}$. It then sends
$x_1^N$.
 %( (w_{1cc}^{(b-1)}, \hat{w}_{2cc}^{(b-1)} ),w_{1cc}^{(b)},w_{1nc}^{(b)}, w_{1p}^{(b)} )$.
Similarly transmitter 2 decodes $\hat{w}_{1cc}^{(b-1)}$, generates $(w_{2cc}^{(b)},w_{2nc}^{(b)}, w_{2p}^{(b)})$ and then sends $x_2^N$.
% \left((\hat{w}_{1c}^{(b-1)}, w_{2c}^{(b-1)} ),w_{2c}^{(b)},w_{2p}^{(b)} \right)$.

\subsection{Decoding}
Each receiver waits until total $B$ blocks have been received and then does \emph{backward decoding}.
Notice that a block index $b$ starts from the last $B$ and ends to $1$. For block $b$, receiver 1 finds the unique indices $(\hat{i},\hat{j},\hat{k}, \hat{l})$ such that for some $m \in [1:2^{N R_{2nc}}]$
\begin{align*}
\begin{split}
\left( u^N ( \hat{i}, \hat{j} ), u_1^N ( ( \hat{i}, \hat{j}) , \hat{w}_{1cc}^{(b)} ), v_1^N ( ( \hat{i}, \hat{j}) , \hat{w}_{1cc}^{(b)}, \hat{k} ),  x_1^N ( (\hat{i}, \hat{j}), \hat{w}_{1cc}^{(b)},  \hat{k}, \hat{l}), \right. \\
 \left. \;\; u_2^N ( (\hat{i}, \hat{j}), \hat{w}_{2cc}^{(b)} ), v_2^N ( (\hat{i}, \hat{j}), \hat{w}_{2cc}^{(b)}, m ) , y_1^{N,(b)}  \right) \in \mathcal{T}_{\epsilon}^{(N)},
\end{split}
\end{align*}
where we assumed that a pair of messages $(\hat{w}_{1cc}^{(b)}, \hat{w}_{2cc}^{(b)})$ was successively decoded from block $(b+1)$. Similarly receiver 2 decodes $(\hat{w}_{1cc}^{(b-1)}, \hat{w}_{2cc}^{(b-1)}, \hat{w}_{2nc}^{(b)}, \hat{w}_{2p}^{(b)})$.

\subsection{Analysis of Probability Error}
By symmetry, we consider the probability of error only for block $b$ and for a pair of transmitter 1 and receiver 1.
We assume that $(w_{1cc}^{(b-1)},w_{2cc}^{(b-1)}, w_{1nc}^{(b)}, w_{1p}^{(b)}) = (1,1,1,1)$ was sent through block $(b-1)$ and block $b$; and there was no backward decoding error from block $B$ to $(b+1)$, i.e., $(\hat{w}_{1cc}^{(b)}, \hat{w}_{2cc}^{(b)})$ are successfully decoded.

Define an event:
\begin{align*}
E_{ijklm} = \left\{ \left( u^N ( i, j ), u_1^N ( ( i, j) , \hat{w}_{1cc}^{(b)} ), v_1^N ( ( i, j) , \hat{w}_{1cc}^{(b)}, k ),  x_1^N ( (i, j), \hat{w}_{1cc}^{(b)},  k, l), \right. \right. \\
 \left. \left. u_2^N ( (i, j), \hat{w}_{2cc}^{(b)} ) , v_2^N ( (i, j), \hat{w}_{2cc}^{(b)}, m ) , y_1^{N,(b)}  \right) \in \mathcal{T}_{\epsilon}^{(N)} \right\}.
\end{align*}
By AEP, the first type of error becomes negligible. Hence, we focus only on the second type of error. Using the union bound, we get
\begin{align}
\begin{split}
\label{eq-errorprobability}
\textrm{Pr} & \left( \bigcup_{(i,j,k,l)  \neq (1,1,1,1), m } E_{ijklm}   \right)
\leq \underbrace{ \sum_{(i,j) \neq (1,1)} \textrm{Pr} \left( \bigcup_{k,l,m} E_{ijklm} \right)}_{\triangleq \textrm{Pr}(E_1)} +
\underbrace{ \sum_{k \neq 1} \textrm{Pr} \left( \bigcup_{l} E_{11kl1} \right)}_{\triangleq \textrm{Pr}(E_2)} \\
&\qquad \qquad + \underbrace{ \sum_{k \neq 1, m \neq 1} \textrm{Pr} \left( \bigcup_{l} E_{11klm} \right)}_{\triangleq \textrm{Pr}(E_3)} + \underbrace{ \sum_{l \neq 1} \textrm{Pr} \left( E_{111l1} \right)}_{\triangleq \textrm{Pr}(E_4)}
+ \underbrace{ \sum_{l \neq 1, m \neq 1 } \textrm{Pr} \left( E_{111lm} \right)}_{\triangleq \textrm{Pr}(E_5)} \\
& \leq 24 \times 2^{N(R_{1cc}+ R_{2cc}+ R_{1nc} + R_{2nc} + R_{1p} - I(U,X_1,V_2;Y_1)+ 5 \epsilon)} \\
& +2 \times 2^{N(R_{1nc}+R_{1p} - I(X_1;Y_1|U,U_1,V_2)+  2 \epsilon)} + 2\times 2^{N(R_{1nc}+ R_{2nc} + R_{1p} - I(X_1, V_2 ;Y_1|U,U_1, U_2)+ 3 \epsilon)} \\
 &+ 2^{N(R_{1p} - I(X_1;Y_1|U,V_1,V_2)+  \epsilon)}  +2^{N(R_{2nc} + R_{1p} - I(X_1,V_2;Y_1|U,V_1, U_2)+ 2 \epsilon)}.
\end{split}
\end{align}

From (\ref{eq-R2c-constraint}) and (\ref{eq-errorprobability}), the error probability can be made arbitrarily small if
\begin{align}
&\left\{
  \begin{array}{ll}
    R_{2cc} &\leq \min(I(U_2;Y_1|U,X_1),C_{\sf FB1} - \delta_1 ) \\
    R_{1p} &\leq I (X_1; Y_1| U, V_1, V_2) \\
    R_{1p} + R_{2nc} &\leq I(X_1,V_2;Y_1|U,V_1, U_2)  \\
    R_{1p} + R_{1nc} &\leq I(X_1;Y_1|U,U_1, V_2)  \\
   R_{1p} + R_{1nc} + R_{2nc} &\leq I(X_1,V_2;Y_1|U,U_1, U_2) \\
   R_{1p} + R_{1cc} + R_{2cc} +  R_{1nc} + R_{2nc} &\leq I(U, V_2, X_1;Y_1) \\
  \end{array}
\right. \\
&\left\{
   \begin{array}{ll}
    R_{1cc} &\leq \min ( I(U_1;Y_2|U,X_2), C_{\sf FB2}- \delta_2 ) \\
    R_{2p} &\leq I (X_2; Y_2| U, V_1, V_2) \\
    R_{2p} + R_{1nc} &\leq I(X_2,V_1;Y_2|U,V_2, U_1) \\
    R_{2p} + R_{2nc} &\leq I(X_2;Y_2|U,U_2, V_1) \\
   R_{2p} + R_{2nc} + R_{1nc} &\leq I(X_2,V_1;Y_2|U,U_1, U_2) \\
   R_{2p} + R_{2cc} + R_{1cc} +  R_{1nc} + R_{2nc} &\leq I(U, V_1, X_2;Y_2) \\
  \end{array}
\right.
%&R_{2c} \leq H(Y_1|X_1,V_1,U) \\
%& R_{1p} \leq H(Y_1|V_1,V_2,U) \\
%& R_{1p}+ R_{2c} \leq C_0 + H(Y_1|V_1,U) \\
%&R_{1c}+R_{1p} \leq C_0 + H(Y_1|V_2,U) \\
%&R_{1c}+R_{1p}+R_{2c} \leq C_0 + H(Y_1|U).
\end{align}

==> GaussianAch.tex <==
\begin{itemize}

\item Case $2_b$:

In this case the basic idea behind our scheme is interference avoidance, \emph{i.e.} each transmitter will maximize its rate as long its signal is received below the noise level at the unintended receiver. Through using feedback, we will be able to go beyond this sum-rate. We consider the case where $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$.

At the beginning of each block, transmitter $1$ independently generates three transmit signals, \emph{i.e.} $X_1^{(1)}, X_1^{(2)}$ and $X_1^{(3)}$. To create these transmit signals, the following set of constraints are ought to be satisfied: 
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
&P_1 = P_1^{(1)} + P_1^{(2)} + P_1^{(3)} \leq 1\\
&P_1^{(1)} + P_1^{(2)} = \min(\frac{1}{\sf INR_{12}},1)
\end{array} \right.
\end{equation}
these conditions are required for the decodability of messages.

Transmitter $2$ independently generates two transmit signals, \emph{i.e.} $X_2^{(1)}$ and $X_2^{(2)}$. We assign power levels at transmitter $2$ such that
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
&P_2 = P_2^{(1)} + P_2^{(2)} \leq 1\\
&P_2^{(1)} = \min(\frac{1}{\sf INR_{21}},1)
\end{array} \right.
\end{equation}
and we also set the power levels such that ${\sf SNR_1} P_1^{(1)} = {\sf INR_{21}} P_2^{(2)} = 2^{C_{\sf FB}} - 1$. In other words, we want $X_1^{(1)}$ and $X_2^{(2)}$ to be received at the same power level at receiver $1$, so that they create a valid lattice point together.

Assume that $X_1^{(3)}$ does not exist ($X_1^{(3)}$ will be the repetition of $X_2^{(2)}$ during the following block) and as a result $X_1^{(2)}$ has the highest power at transmitter $1$ and it should be decodable at receiver $1$ treating other signals as noise.
\begin{equation}
R_1^{(2)} \leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} P_1^{(1)}} \right)
\end{equation}

At the end of a block, receiver $1$ will decode and remove $X_1^{(2)}$ from the received signal. Now, receiver $1$ should be able to decode $X_1^{(1)}$ interfered by $X_2^{(2)}$. Receiver $1$ will send back the lattice index of the interfered signal through the feedback link (this can be done as long as $R_2^{(2)} \leq C_{\sf FB}$ \cite{twoway}, which justifies ${\sf INR_{21}} P_2^{(2)} = 2^{C_{\sf FB}} - 1$). These are reflected in the following constraints imposed on $R_1^{(1)}$ and $R_2^{(2)}$:
\begin{equation}
\begin{split}
R_1^{(1)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right)\\
R_2^{(2)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right)
\end{split}
\end{equation}

At the beginning of each block (with the exception of the first block), transmitter $1$ will receive a lattice index through the feedback link from which it can decode the interfering message coming from transmitter $2$, also note that this is the interference that has occured in the previous block. The interfering message will be decoded and then encoded as $X_1^{(3)}$; since this message is already known to receiver $2$, it can be easily removed from the received signal and as a result it will not cause interference at receiver $2$. However, $X_1^{(3)}$ should be decodable at receiver $1$:
\begin{equation}
R_1^{(3)} \leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(3)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} ( P_1^{(1)} + P_1^{(2)} ) } \right)
\end{equation}

In order to carry out the decoding scheme at receiver $2$ with arbitrary small error probability, the following constraints should be satisfied.
\begin{equation}
\begin{split}
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} ) } \right)\\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf SNR_2} P_2^{(1)} + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} ) } \right) 
\end{split}
\end{equation}

The arugument presented above describes a set of constraints on the rates, which is summerized as follows:
\begin{equation}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} P_1^{(1)}} \right) \\
R_1^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(3)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} ( P_1^{(1)} + P_1^{(2)} ) } \right) \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} ) } \right)\\
R_2^{(2)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right) \\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf SNR_2} P_2^{(1)} + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} ) } \right)
\end{array} \right.
\end{equation}
note that $X_1^{(3)}$ is in fact the repetition of $X_2^{(2)}$ and as a result it should not considered as part of $R_1$ when calculating the achievable sum-rate. We can simplify this result by removing the loose upper-bound on $R_2^{(2)}$:
\begin{equation}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} P_1^{(1)}} \right) \\
R_1^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(3)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} ( P_1^{(1)} + P_1^{(2)} ) } \right) \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} ) } \right)\\
R_2^{(2)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right) \\
\end{array} \right.
\end{equation}

A similar achievability scheme works for the other extreme case, \emph{i.e.} $C_{\sf FB1} = 0$ and $C_{\sf FB2} = C_{\sf FB}$. At the beginning of each block, transmitter $2$ independently generates three transmit signals, \emph{i.e.} $X_2^{(1)}, X_2^{(2)}$ and $X_2^{(3)}$. To create these transmit signals, the following set of constraints are ought to be satisfied: 
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
&P_2 = P_2^{(1)} + P_2^{(2)} + P_2^{(3)} \leq 1\\
&P_2^{(1)} + P_2^{(2)} = \min(\frac{1}{\sf INR_{21}},1)
\end{array} \right.
\end{equation}
these conditions are required for the decodability of messages.

Transmitter $1$ independently generates two transmit signals, \emph{i.e.} $X_1^{(1)}$ and $X_1^{(2)}$. We assign power levels at transmitter $1$ such that
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
&P_1 = P_1^{(1)} + P_1^{(2)} \leq 1\\
&P_1^{(1)} = \min(\frac{1}{\sf INR_{12}},1)
\end{array} \right.
\end{equation}
and we also set the power levels such that ${\sf SNR_2} P_2^{(1)} = {\sf INR_{12}} P_1^{(2)} = 2^{C_{\sf FB}} - 1$. In other words, we want $X_2^{(1)}$ and $X_1^{(2)}$ to be received at the same power level at receiver $2$, so that they create a valid lattice point together.

Assume that $X_2^{(3)}$ does not exist ($X_2^{(3)}$ will be the repetition of $X_1^{(2)}$ during the following block) and as a result $X_2^{(2)}$ has the highest power at transmitter $2$ and it should be decodable treating other signals as noise at receiver $2$.
\begin{equation}
R_2^{(2)} \leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf INR_{12}} P_1 + {\sf SNR_2} P_2^{(1)}} \right)
\end{equation}

At the end of a block, receiver $2$ will decode and remove $X_2^{(2)}$ from the received signal. It has now access to $X_2^{(1)}$ interfered by $X_1^{(2)}$. Receiver $2$ will send back the lattice index of the interfered signal through the feedback link (this can be done as long as $R_1^{(2)} \leq C_{\sf FB}$ \cite{twoway}, which justifies ${\sf INR_{12}} P_1^{(2)} = 2^{C_{\sf FB}} - 1$). These are reflected in the following constraints imposed on $R_2^{(1)}$ and $R_1^{(2)}$:
\begin{equation}
\begin{split}
R_1^{(2)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf INR_{12}} P_1^{(2)}}{1 + {\sf INR_{12}} P_1^{(1)}} \right) \\
R_2^{(1)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} P_1^{(1)}} \right)
\end{split}
\end{equation}

At the beginning of each block (with the exception of the first block), transmitter $2$ will receive a lattice index through the feedback link from which it can decode the interfering message coming from transmitter $1$, also note that this is the interference that has occured in the previous block. The interfering message will be decoded and then encoded as $X_2^{(3)}$; since this message is already known to receiver $2$, it can be easily removed from the received signal and as a result it will not cause interference at receiver $1$. However, $X_2^{(3)}$ should be decodable at receiver $2$:
\begin{equation}
R_2^{(3)} \leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(3)}}{1 + {\sf INR_{12}} P_1 + {\sf SNR_2} ( P_2^{(1)} + P_2^{(2)} ) } \right)
\end{equation}

In order to carry out the decoding scheme at receiver $1$ with arbitrary small error probability, the following constraints should be satisfied.
\begin{equation}
\begin{split}
R_1^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} ( P_2^{(1)} + P_2^{(2)} ) } \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf SNR_1} P_1^{(1)} + {\sf INR_{21}} ( P_2^{(1)} + P_2^{(2)} ) } \right) 
\end{split}
\end{equation}

The arugument presented above describes a set of constraints on the rates, keeping only the effective upper-bounds we get:
\begin{equation}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} ( P_2^{(1)} + P_2^{(2)} ) } \right)\\
R_1^{(2)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf INR_{12}} P_1^{(2)}}{1 + {\sf INR_{12}} P_1^{(1)}} \right) \\
R_2^{(1)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} P_1^{(1)}} \right)\\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf INR_{12}} P_1 + {\sf SNR_2} P_2^{(1)}} \right) \\
R_2^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(3)}}{1 + {\sf INR_{12}} P_1 + {\sf SNR_2} ( P_2^{(1)} + P_2^{(2)} ) } \right) 
\end{array} \right.
\end{equation}
note that $X_2^{(3)}$ is in fact the repetition of $X_1^{(2)}$ and as a result it should not considered as part of $R_2$ when calculating the achievable sum-rate. For any other feedback assignment a time sharing of the two extreme cases will provide us with the sum-rate we are looking for.

\item Case $2_c$:

The achievability scenario in this case is very similar to that of case $1_b$ except that an extra $X_1^{(4)}$ will be required at transmitter $1$. The decodability works in a similar manner to those presented for $1_a$ and $1_b$ and as a result its eliminated. Again we consider $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$ and the other extreme case follows naturally. 

The scheme will result in a set of constraints on the rates, which is summerized as follows.
\begin{equation}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} P_1^{(1)}} \right) \\
R_1^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(3)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} ( P_1^{(1)} + P_1^{(2)} ) } \right) \\
R_1^{(4)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(4)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} ( P_1^{(1)} + P_1^{(2)} + P_1^{(3)} ) } \right) \\
R_1^{(4)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(4)}}{1 + {\sf SNR_2} P_2^{(1)} + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} ) } \right) \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} ) } \right)\\
R_2^{(2)} &\leq \log \left( \frac{1}{2} + \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)}} \right) \\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf SNR_2} P_2^{(1)} + {\sf INR_{12}} ( P_1^{(1)} + P_1^{(2)} + P_1^{(4)} ) } 
\end{array} \right.
\end{equation}
note that $X_1^{(3)}$ is in fact the repetition of $X_2^{(2)}$ and as a result it should not considered as part of $R_1$ when calculating the achievable sum-rate.

Now what happens if the first outer-bound, \emph{i.e.} $R_1 + R_2 \leq \log \left( 1 +  \frac{ (1- \rho^2) \mathsf{SNR}_1}{ 1 + (1- \rho^2) \mathsf{INR}_{12}} \right) +  \log \left( 1+ \mathsf{SNR}_2  + \mathsf{INR}_{12} + 2 \rho \sqrt{ \mathsf{SNR}_2  \cdot \mathsf{INR}_{12}} \right) $, is tighter? There two scenraios possible, if we set $C_{\sf FB1} = C_{\sf FB2} = 0$ and this outer-bound is still tighter then feedback cannot help us to increase sum-rate and as a result we can use the achievability scheme develpoped in \cite{Etkin}. Otherwise, one of the cases $1_a$, $1_b$ or $1_c$ is tighter and we will use the feedback capacity till the point where the other outer-bound becomes active, beyond this point feedback cannot help us to increase the capacity.

\item Case $3$:

As we can see in table~\ref{table:Gaussian} in case $3$, \emph{i.e.} $ \log \left( {\sf SNR_2 } \right) \geq \log \left( {\sf SNR_1 } \right) \geq \log \left( {\sf INR_{12} } \right) \geq \log \left( {\sf INR_{21} } \right)$, feedback can help also us increase sum-rate compared to the non-feedback scenario. The achievability scheme is going to be similar to those presented for case $1$ and are removed for the sake of simplicity.

\end{itemize}

%%%%%%%%%%%%%%%%% typing %%%%%%%%%%%%%%%%%%%%%%

\item {\bf Strong Interference}:

We define the strong interference regime by the following inequalities
\begin{equation}
\label{}
\nonumber
\begin{split}
\log \left( {\sf INR_{12} } \right) \geq \log \left( {\sf SNR_1 } \right)\\
\log \left( {\sf INR_{21} } \right) \geq \log \left( {\sf SNR_2 } \right)
\end{split}
\end{equation}

As for the weak interference regime, we only consider cases where feedback can help us increase the sum-rate. There are a total of four cases to study, however we only need to study two cases since the other three will simply follow by interchanging the transmitter-receiver pairs' \emph{id}'s, see Table~\ref{table:Gaussian}.
\begin{equation}
\label{}
\begin{split}
5: \hspace{4mm} \log \left( {\sf INR_{21} } \right) \geq \log \left( {\sf INR_{12} } \right) \geq \log \left( {\sf SNR_2 } \right) \geq \log \left( {\sf SNR_1 } \right) \\
6: \hspace{4mm} \log \left( {\sf INR_{21} } \right) \geq \log \left( {\sf INR_{12} } \right) \geq \log \left( {\sf SNR_1 } \right) \geq \log \left( {\sf SNR_2 } \right) 
\end{split}
\end{equation}

The effective upper bounds on sum-rate in these two cases are:
\begin{align}
\label{eq:strong1}
R_1 + R_2 &\leq \log \left( 1 +  (1- \rho^2) \mathsf{SNR}_1 \right) + \log \left( 1 +  (1- \rho^2) \mathsf{SNR}_2 \right) + C_{\sf FB1 } + C_{\sf FB2 }\\
R_1 + R_2 &\leq \log \left( 1 +  \frac{ (1- \rho^2) \mathsf{SNR}_1}{ 1 + (1- \rho^2) \mathsf{INR}_{12}} \right) +  \log \left( 1+ \mathsf{SNR}_2  + \mathsf{INR}_{12} + 2 \rho \sqrt{ \mathsf{SNR}_2  \cdot \mathsf{INR}_{12}} \right)
\end{align}

\begin{itemize}

\item Case $5$:

Either of these outer-bounds can be the effective one, we will present our achievability strategy in each case separately. Assume that due to channel gains, the first outer-bound is tighter, we can consider two extreme cases: $C_{\sf FB1} = 0$ or $C_{\sf FB2} = 0$. The achievability strategy will be very similar in either case and as a result, we will only describe the achievability scheme for the former one. 

At the beginning of each block transmitter $1$ independently generates two transmit signals, \emph{i.e.} $X_1^{(1)}$ and $X_1^{(2)}$. We set the power assignment such that it satisfies the following conditions.
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
&P_1 = P_1^{(1)} + P_1^{(2)} \leq 1\\
&P_1^{(1)} = \min(\frac{1}{\sf SNR_1},1)
\end{array} \right.
\end{equation}

Transmitter $2$ will also independently generate two transmit signals, \emph{i.e.} $X_2^{(1)}$ and $X_2^{(2)}$. We assign power levels at transmitter $2$ such that
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
&P_2 = P_2^{(1)} + P_2^{(2)} \leq 1\\
&P_2^{(1)} = \min(\frac{1}{\sf SNR_2},1)
\end{array} \right.
\end{equation}

Due to the assumptions we have made, at each receiver the signal from interfering transmitter will be received at a higher power level than the signal from intended transmitter. For simplicity of description assume that $X_1^{(1)}$ does not exist (as it will be clear later $X_1^{(1)}$ is part of the message intended for receiver $2$), therefore $X_1^{(2)}$ is the only signal transmitted from transmitter $1$. Receiver $1$ will first decode the signal coming from transmitter $2$, treating other signals as noise. Receiver $1$ will decode $X_2^{(2)}$ and will remove it from the recived signal. Decoding wii be carried on by decoding $X_2^{(1)}$. This requires
\begin{equation}
\begin{split}
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf INR_{21}} P_2^{(1)}}{1 + {\sf SNR_1} P_1^{(2)}} \right)\\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)} + {\sf SNR_1} P_1^{(2)} } \right)
\end{split}
\end{equation}

Reciver $1$ will send back the lattice index of $X_2^{(1)}$ back to transmitter $1$ through the feedback link and transmitter $1$ will encode it as $x_1^{(1)}$ (as described before, we should be aware of the fact that $X_1^{(1)}$ in each block is actually the message received from transmitter $2$ during the previous block). This requires
\begin{equation}
R_2^{(1)} \leq C_{\sf FB}
\end{equation}

A main difference in the strong interference case in comparison to the weak interference case is that we do not use feedback in order to resolve interference, but to provide the other receiver with part of its intended message that is not directly available to it. In other words, we are creating an additional path in the network, for example in this case the new path is transmitter $2$ $\rightarrow$ receiver $1$ $\rightarrow$ transmitter $1$ $\rightarrow$ receiver $2$. 

Receiver $2$ will first decode the message coming from transmitter $1$, note that part of this message is in fact intended for receiver $2$. 
\begin{equation}
\begin{split}
R_1^{(1)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(1)}}{1 + {\sf SNR_2} P_2} \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(2)}}{1 + {\sf INR_{12}} P_1^{(1)} + {\sf SNR_2} P_2 } \right)
\end{split}
\end{equation}

Finally, each receiver should be able to decode its intended message coming from its own transmitter. This can be accomplished with arbitrary small error probability if
\begin{equation}
\begin{split}
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf SNR_1} P_1^{(1)}} \right)\\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf SNR_2} P_2^{(1)} } \right)
\end{split}
\end{equation}

The following set of inequalities summerizes the achievable sum-rate through our strategy.
\begin{equation}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(1)}}{1 + {\sf SNR_2} P_2} \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf SNR_1} P_1^{(1)}} \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(2)}}{1 + {\sf INR_{12}} P_1^{(1)} + {\sf SNR_2} P_2 } \right)\\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf INR_{21}} P_2^{(1)}}{1 + {\sf SNR_1} P_1} \right)\\
R_2^{(1)} &\leq C_{\sf FB}\\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)} + {\sf SNR_1} P_1 } \right)\\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf SNR_2} P_2^{(1)} } \right)
\end{array} \right.
\end{equation}
note that $R_1^{(2)}$ does not convey a new message and as a result should not be considered as a part of $R_1$ when calculating the sum-rate. These inequalities can be further simplified by removing the loose bounds as follows:
\begin{equation}
\left\{ \begin{array}{ll}
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf SNR_1} P_1^{(1)}} \right)\\
R_1^{(2)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(2)}}{1 + {\sf INR_{12}} P_1^{(1)} + {\sf SNR_2} P_2 } \right)\\
R_2^{(1)} &\leq C_{\sf FB}\\
R_2^{(2)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf SNR_2} P_2^{(1)} } \right)
\end{array} \right.
\end{equation}


Now consider the case where the second outer-bound 
$$ \log \left( 1 +  \frac{ (1- \rho^2) \mathsf{SNR}_1}{ 1 + (1- \rho^2) \mathsf{INR}_{12}} \right) +  \log \left( 1+ \mathsf{SNR}_2  + \mathsf{INR}_{12} + 2 \rho \sqrt{ \mathsf{SNR}_2  \cdot \mathsf{INR}_{12}} \right) $$
is tighter. If by setting $C_{\sf FB1} = C_{\sf FB2} = 0$ this outer-bound is still tighter, then feedback cannot help us increase the sum-rate and we use the achievability scheme developed in~\cite{Etkin}. Otherwise, the achievability is similar to that of the previous case and if we assume that $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$, then transmitter $2$ will transmit at a rate of $\log \left( 1 + {\sf SNR_2 } \right) + C_{\sf FB}$ and the rate from transmitter $1$ will be limited due to the active outer-bound.

\item Case $6$:

Achievability scheme is very similar to case $5$, hence it is not presented.

\end{itemize}

\item {\bf Mix Interference}:

As it is evident from Table~\ref{table:Gaussian}, feedback cannot increase sum-rate in this regime.


\end{itemize}

==> determinitictable.tex <==
Before proceeding to the Gaussain case and presenting our contributions in that case, it is worth investigating our presented results a little bit more and compare it with existing results.

\begin{remark}
\label{remark:ISIT}

In \cite{AlirezaISIT}, we fully characterized the sum-rate capacity of the symmetric two-user linear deterministic interference channel with rate-limited feedback. That result is a special case of our current result and it can be recovered from Theorem~\ref{theorem:DICcapacity} by setting $n_{11} = n_{22} = n$, $n_{12} = n_{21} = m$ and $C_{\sf FB1} = C_{\sf FB2} = R_f$. In \cite{AlirezaISIT}, our main message was that for the network we considered \emph{one bit} of feedback can at most increase the sum-rate capacity by \emph{one bit}. In the current correspondence, we have taken a step further and and we have shown that ``one bit of feedback is at most worth one bit in the capacity region of any deterministic (that is a subset of El Gamal-Costa model) two-user interference network''. 

\end{remark}

\begin{remark}
\label{remark:comparison}

It is completely natural that one expects the capacity region of the two-user deterministic IC with rate-limited feedback contains that of the two-user deterministic IC with no feedback~\cite{Etkin} and is included by the capacity region of the two-user deterministic IC with infinite feedback~\cite{Suh}. This intuitive result can be best depicted in terms of sum-rate capacity when we consider symmetric parameters~\cite{Alireza:ISIT}, see Figure~\ref{symmetric-curve} for a depiction.

\begin{figure}[ht]
\centering
\includegraphics[width=8.4cm,height=5cm]{p8.jpg}
\caption{A comparison: limited feedback vs. infinite feedback and non-feedbacl.}
\end{figure}

\end{remark}

\begin{remark}

In the following section we focus on sum-rate capacity of the two-user Gaussian IC with rate limited feedback. It is a known fact that linear deterministic model provides us with great insights about the Gaussian model~\cite{}. From Theorem~\ref{theorem:DICcapacity}, we can extract cases where feedback indeed increases sum-rate capacity of the linear deterministic model compared to that of the non-feedback case. These are the cases where we can also have hopes to increase the sum-rate in the Gaussian case. Table~\ref{table:linear} summerizes these cases. Weak interference regime is characterized by $n_{12} \leq n_{11}$ and $n_{21} \leq n_{22}$, whereas the strong interference regime refers to all cases where $n_{12} \geq n_{11}$ and $n_{21} \geq n_{22}$. Any case that is strong or weak is considered as mix interference regime. A ``$+$'' sign in this table indicates the fact that feedback increases the sum-rate capacity of the network compared to that of the non-feedback case. Also note that we have a total of $24$ cases however, we have only $12$ cases presented in Table~\ref{table:linear}; this is due to the fact that the other $12$ cases can be obtained by simply interchanging the pairs' \emph{id}'s.

\begin{table}[h]
\caption{}
\centering
\begin{tabular}{| c | c | c | c | c | c | c |}
\hline
Case \emph{id}	& regime  &	 & $B_1$    & $B_2$		& $B_3$		& $B_4$ \\
%heading
\hline
$1$ & weak  & $n_{11} \geq n_{12} \geq n_{22} \geq n_{21}$  & - & - & - & - \\
\hline
$2$ & weak  & $n_{11} \geq n_{22} \geq n_{12} \geq n_{21}$  & - & + & - & + \\
\hline
$3$ & weak  & $n_{22} \geq n_{11} \geq n_{12} \geq n_{21}$  & - & + & - & + \\
\hline
$4$ & strong  & $n_{21} \geq n_{22} \geq n_{12} \geq n_{11}$  & - & - & - & - \\
\hline
$5$ & strong  & $n_{21} \geq n_{12} \geq n_{22} \geq n_{11}$  & + & + & - & - \\
\hline
$6$ & strong  & $n_{21} \geq n_{12} \geq n_{11} \geq n_{22}$  & + & + & - & - \\
\hline
$7$ & mix  & $n_{11} \geq n_{12} \geq n_{21} \geq n_{22}$  & - & - & - & - \\
\hline
$8$ & mix  & $n_{11} \geq n_{21} \geq n_{12} \geq n_{22}$  & - & - & - & - \\
\hline
$9$ & mix  & $n_{11} \geq n_{21} \geq n_{22} \geq n_{12}$  & - & - & - & - \\
\hline
$10$ & mix  & $n_{21} \geq n_{11} \geq n_{12} \geq n_{22}$  & - & - & - & - \\
\hline
$11$ & mix  & $n_{21} \geq n_{22} \geq n_{11} \geq n_{12}$  & - & - & - & - \\
\hline
$12$ & mix  & $n_{21} \geq n_{11} \geq n_{22} \geq n_{12}$  & - & - & - & - \\
\hline
\end{tabular}
\label{table:linear}
\end{table}

\end{remark}

==> equivalent.tex <==
We will show that the inequalities developed in the proof of Theorem~\ref{theorem:DICcapacity} are equivalent to the capacity region in Theorem~\ref{theorem:DICcapacity}. Note that (\ref{eq2:R1bound-2}) can be written as
\begin{align*}
R_1 \leq \left\{
  \begin{array}{ll}
n_{11} + C_{\sf FB2}, & \hbox{ $n_{11} + C_{\sf FB2} \leq n_{12}$;} \\
    \max( n_{11}, n_{12}),
& \hbox{otherwise.}
  \end{array}
\right.
\end{align*}
This shows that this inequality is implied by (\ref{eq:R1bound-1}) and (\ref{eq:R1bound-2}). Similarly, (\ref{eq2:R2bound-2}) is implied by (\ref{eq:R2bound-1}) and (\ref{eq:R2bound-2}).
Next consider (\ref{eq2:R1R2bound-3}):
\begin{align*}
R_1 +R_2 \leq \left\{
  \begin{array}{ll}
\max \left \{ (n_{11}-n_{12})^+,  n_{21} \right \}  +  \max \left \{ (n_{22}-n_{21})^+, n_{12} \right \}  + C_{\sf FB1} + C_{\sf FB2}, \\
\qquad \qquad  \hbox{ if $C_{\sf FB1} \leq \min \left\{ (n_{11} - n_{12})^+, n_{21} \right\}$, $C_{\sf FB2} \leq \min \left\{ (n_{22} - n_{21})^+, n_{12} \right\}$;} \\
    \max( n_{11}, n_{12}) + \max( n_{21}, n_{22}), \\
\qquad \qquad  \hbox{ if $C_{\sf FB1} > \min \left\{ (n_{11} - n_{12})^+, n_{21} \right\}$, $C_{\sf FB2} > \min \left\{ (n_{22} - n_{21})^+, n_{12} \right\}$;} \\
  \max \left \{ (n_{11}-n_{12})^+,  n_{21} \right \} + C_{\sf FB1} + n_{12}
  + (n_{22}-n_{21})^+, \\
\qquad \qquad  \hbox{ if $C_{\sf FB1} \leq \min \left\{ (n_{11} - n_{12})^+, n_{21} \right\}$, $C_{\sf FB2} > \min \left\{ (n_{22} - n_{21})^+, n_{12} \right\}$;} \\
  \max \left \{ (n_{22}-n_{21})^+,  n_{12} \right \} + C_{\sf FB2} + n_{21}
  + (n_{11}-n_{12})^+, \\
\qquad \qquad  \hbox{ if $C_{\sf FB1} > \min \left\{ (n_{11} - n_{12})^+, n_{21} \right\}$, $C_{\sf FB2} \leq \min \left\{ (n_{22} - n_{21})^+, n_{12} \right\}$.}
  \end{array}
\right.
\end{align*}
Note that the first case is implied by (\ref{eq:R1R2bound-3}); and the second case is implied by (\ref{eq:R1bound-1}) and (\ref{eq:R2bound-1}). Also notice that the third case is implied by (\ref{eq:R2bound-1}) and (\ref{eq:R12R2bound}); and the last case is implied by  (\ref{eq:R1bound-1}) and (\ref{eq:2R1R2bound}). Lastly, we consider (\ref{eq2:2R1R2bound}):
\begin{align*}
2R_1 +R_2 \leq \left\{
  \begin{array}{ll}
(n_{11} - n_{12})^+  +  \max( n_{11}, n_{21}) +  \max \left \{ (n_{22}-n_{21})^+,  n_{12}  \right \} + C_{\sf FB2}, \\
\qquad \qquad  \hbox{ if $C_{\sf FB2} \leq \min \left\{ (n_{22} - n_{21})^+, n_{12} \right\}$;} \\
    \max ( n_{11}, n_{12})  +  \max( n_{11}, n_{21}) +  (n_{22}-n_{21})^+, \\
\qquad \qquad  \hbox{ if $C_{\sf FB2} > \min \left\{ (n_{22} - n_{21})^+, n_{12} \right\}$.}
  \end{array}
\right.
\end{align*}
Note that the first case is implied by (\ref{eq:2R1R2bound}); and the second case is implied by (\ref{eq:R1bound-1}) and (\ref{eq:R1R2bound-2}).
Similarly, it can be shown that (\ref{eq2:R12R2bound}) is implied by (\ref{eq:R12R2bound}), (\ref{eq:R2bound-1}) and (\ref{eq:R1R2bound-1}). Therefore, the inequalities of (\ref{eq2:R1bound-1})-(\ref{eq2:R12R2bound}) are equivalent to those of (\ref{eq:R1bound-1})-(\ref{eq:R12R2bound}), thus proving the achievablity of Theorem~\ref{theorem:DICcapacity}.

==> gaussian-symmetric.tex <==
In this section, we consider the two-user Gaussian IC with rate-limited feedback. The Gaussian model is described in section~\ref{problem}. For most of this paper, we focus on the symmetric two-user Gaussian IC (except for the outer bound) and assume that
\begin{equation}
\begin{split}
& h_{11} = h_{22} = h_d, \\
& h_{12} = h_{21} = h_c, 
\end{split}
\end{equation}
and
\begin{equation}
\begin{split}
& {\sf SNR}_1 = {\sf SNR}_2 = {\sf SNR} = |h_d|^2, \\
& {\sf INR}_{12} = {\sf INR}_{21} = {\sf INR} = |h_c|^2. 
\end{split}
\end{equation}

The following theorem is our main result in this section.

\begin{theorem} \label{THM:Gaussian-sumrate}
The sum-rate capacity of the two-user Gaussian IC with rate-limited feedback is within at most $9.8$ bits/sec/Hz of the maximum $R_1 + R_2$ satisfying
\begin{subequations}
\begin{eqnarray}
\label{eq:sum1}
0 \leq R_1 + R_2 & \leq & 2 \log \left( 1 + \mathsf{SNR} \right) + C_{\sf FB1 } + C_{\sf FB2 } \\
\label{eq:sum2}
0 \leq R_1 + R_2 & \leq & \log \left( 1 +  \frac{  \mathsf{SNR}}{ 1 +  \mathsf{INR}} \right) \\
& + &  \log \left( 1+ \mathsf{SNR} + \mathsf{INR} + 2 \sqrt{ \mathsf{SNR}  \cdot \mathsf{INR}} \right) \nonumber \\
\label{eq:sum4}
0 \leq R_1 + R_2 & \leq & 2 \log \left( 1 + {\sf INR} + \frac{ {\sf SNR} }{1+ {\sf INR}} \right) \\
& + & \min \{ C_{\sf FB1}, \log \left( 1 + \mathsf{INR} \right) \} \nonumber \\
& + & \min \{ C_{\sf FB2}, \log \left( 1 + \mathsf{INR} \right) \} \nonumber
\end{eqnarray}
\end{subequations}
\end{theorem}

In Appendix~\ref{Appendix:Gaussian}, we present an outer-bound on the capacity region of the general two-user Gaussian interference channel with rate-limited feedback (i.e., not necessarily symmetric). The converse for Theorem~\ref{THM:Gaussian-sumrate} is then a direct result of Theorem~\ref{theorem:Gaussianouterbound} in Appendix C. The rest of this section is dedicated to describing the achievability scheme.

We first provide a brief outline of the achievability. Our achievability scheme is a based on Block Markov coding, where we use backward decoding at the receivers. The scheme is implemented over $B$ blocks. In each block (with the exception of the last two), new messages are transmitted. At the end of a block, each receiver creates a feedback message according to our feedback strategy and sends it back to its corresponding transmitter. This will provide each transmitter with part (or all) of the interference from the other user. Each transmitter encodes this interfering message and transmit it to its receiver during a different block. Through this part of the transmit signal, receivers will be able to complete the decoding of the previously received messages. During the last two blocks, no new messages will be transmitted and each transmitter provides its receiver with the interfering message coming from the other transmitter. Later, we let $B$ go to infinity to achieve our desired result.

As we have seen in Section~\ref{motivation}, each receiver may need to decode the superposition the of codewords corresponding to the cooperative common message of the other transmitter and part of the private message of its transmitter. In order to be able to decode the superposition of codewords in Gaussian model, we use lattice codes as it will be discussed later.

\subsection{Lattice Coding Preliminaries}

In this subsection, we briefly go over some preliminaries on lattice coding and summerize the results that are going to be used in this paper. A lattice is a discrete additive subgroup of $\mathbb{R}^n$. The fundamental volume $V_f(\Lambda)$ of a lattice $\Lambda$ is the reciprocal of the number of lattice points per unit volume.

Given integer $p$, denote the set of integers modulo $p$ by $\mathbb{Z}_p$. Let $\mathbb{Z}^n \rightarrow \mathbb{Z}_p^n: v \mapsto \bar{v}$ be the componentwise modulo $p$ operation over integer vectors. Also, let $C$ denote a linear $(n,k)$ code over $\mathbb{Z}_p$. Then the lattice $\Lambda_C$ defined as
\begin{equation}
\Lambda_C = \{ v \in \mathbb{Z}^n : \bar{v} \in C \},
\end{equation}
is generated with respect to the linear code $C$ (see \cite{lattice} for details). In \cite{lattice}, it has been shown that there exists good lattice codes for point-to-point communication channels, \emph{i.e.} codes that achieve a rate close to the capacity of the channel with arbitrary small decoding error probability. We summerize that result here.

Consider a point-to-point communication scenario over an additive noise channel
\begin{equation}
\label{eq:p2p}
Y = X + Z
\end{equation}
where $X$ is the transmitted signal with power constraint $P$, $Y$ is the received signal and $Z$ is the additive noise process with zero mean and variance $\sigma^2$.

Set $\mathcal{B}$ of linear codes over $\mathbb{Z}_p$ is called balanced if every nonzero element of $\mathbb{Z}_p^n$ is contained in the same number of codes in $\mathcal{B}$. Define $\mathcal{L}_\mathcal{B}$ as
\begin{equation}
\label{eq:L}
\mathcal{L}_\mathcal{B} = \{ \Lambda_C : C \in \mathcal{B} \}.
\end{equation}
based on the aforementioned definitions, we have the following result for lattice coding.

\begin{lemma}[\cite{lattice}]
Consider a single user point-to-point additive noise channel described in (\ref{eq:p2p}). Let $\mathcal{B}$ be a balanced set of linear $(n, k)$ codes over $\mathbb{Z}_p$. Averaged over all lattices from the set $\mathcal{L}_\mathcal{B}$ defined in (\ref{eq:L}), each scaled by $\gamma > 0$ and with a fundamental volume $V$, we have that for any $\delta > 0$, the
average probability of decoding error is bounded by
\begin{equation}
\label{}
\bar{P}_e < (1+\delta) \frac{n\frac{1}{2}\log \left( 2 \pi e \sigma^2 \right)}{V}
\end{equation}
for sufficiently large $p$ and small $\gamma$ such that $\gamma^n p^{n-k} = V$.
\end{lemma}

Proof can be found in \cite{lattice}. The next lemma describes the existence of a good lattice code for a point-to-point AWGN channel.

\begin{lemma}[\cite{lattice}]
\label{lemma:lattice}
Consider a point-to-point additive noise channel described in (\ref{eq:p2p}) such that the transmitter satisfies a power constraint of $P$. Then, we can choose a lattice $\Lambda$ generated using construction A, a shift $s$\footnotemark \footnotetext{Shift $s$ is a vector in $\mathbb{R}^n$ and it is required in order to prove of existence of good lattice codes, see \cite{lattice} for more details.} and a shaping region $S$\footnotemark \footnotetext{We need to consider the intersection of a lattice with some shaping region $S \subset \mathbb{R}^n$ to satisfy the power constraint.} such that the codebook $(\Lambda + s) \cap S$ achieves a rate $R$ with arbitrarily small probability of error if
\begin{equation}
\label{}
R \leq \frac{1}{2} \log \left( \frac{P}{\sigma^2} \right)
\end{equation}
\end{lemma}

In other words, Lemma~\ref{lemma:lattice} describes the existence of a lattice code with sufficient codewords. Proof can be found in \cite{lattice}. 

\begin{remark}
In this paper, we consider complex AWGN channels. Similar to Lemma~\ref{lemma:lattice}, one can show that using lattice codes, a rate of $\log \left( \frac{P}{\sigma^2} \right)$ is achievable in a complex AWGN channel.
\end{remark}

\subsection{Acievability Strategy}
\label{achievability}

In this subsection, we describe the achievability scheme for Theorem~\ref{THM:Gaussian-sumrate}. We assume that ${\sf INR} \geq 1$, since for the case when ${\sf INR} < 1$, by ignoring the feedback and treating interfere as noise, we can achieve a sum-rate of
\begin{align}
\label{}
2 \log \left( 1 + \frac{\sf SNR}{1 + {\sf INR}} \right)
\end{align}
which is at most within $2.6$ bits of outerbound (\ref{eq:sum2}) in Theorem~\ref{THM:Gaussian-sumrate}:
\begin{align}
\label{}
&\; \log \left( 1 +  \frac{  \mathsf{SNR}}{ 1 +  \mathsf{INR}} \right) +  \log \left( 1+ \mathsf{SNR} + \mathsf{INR} + 2 \sqrt{ \mathsf{SNR}  \cdot \mathsf{INR}} \right) \nonumber \\
&\; - 2 \log \left( 1 + \frac{\sf SNR}{1 + {\sf INR}} \right) \nonumber \\
&\; \overset{({\sf INR} \leq 1)}{\leq} \log \left( 1+ \mathsf{SNR} + \mathsf{INR} + 2 \sqrt{ \mathsf{SNR}  \cdot \mathsf{INR}} \right) \nonumber \\
&\; - \log \left( 1 + \frac{\sf SNR}{2} \right) \nonumber \\
&\; \overset{({\sf INR} \leq 1)}{\leq} \log \left( 2 + 3 \mathsf{SNR} \right) - \log \left( 1 + {\sf SNR} \right) + 1 \nonumber \\
&\; = \log \left( \frac{2 + 3 \mathsf{SNR}}{1 + {\sf SNR}} \right) + 1 \nonumber \\
&\; \leq \log \left( 3 \right) + 1 \leq 2.6
\end{align}

Moreover, we first describe our strategy for the extreme case where $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$ (or symmetrically $C_{\sf FB2} = C_{\sf FB}$ and $C_{\sf FB1} = 0$). Our strategy for any other feedback configuration will be based on a combination of the strategies for these extreme cases.

\noindent {\bf 1) Codebook Generation and Encoding}

The communication strategy consists of $B$ blocks, each of length $N$ channel uses. In block $b$, $b = 1,2,\ldots,B-2$, transmitter $1$ has $4$ messages $W_1^{(1,b)}, W_1^{(2,b)}, W_1^{(3,b)}$ and $W_1^{(4,b)}$ for receiver $1$, where $W_1^{(i,b)} \in \{ 1, 2, \ldots, 2^{N R_1^{(i)}} \}$. Out of these four messges $W_1^{(1,b)}, W_1^{(2,b)}$ and $W_1^{(4,b)}$ are new messages. We further describe $W_1^{(3,b)}$ when we describe the feedback strategy. On the other hand, transmitter $2$ has $3$ new independent messages $W_2^{(1,b)}, W_2^{(2,b)}$ and $W_2^{(3,b)}$ for receiver $2$.

At transmitter $k$, message $W_k^{(i,b)}$ is mapped to $X_k^{(i,b)}$, where $X_k^{(i,b)}$ is a Gaussian codeword pricked from a codebook of size $2^{N R_k^{(i)}}$ and any elemnet of this codebook is distributed as i.i.d. $\mathcal{CN}(0,P_k^{(i)})$, $(k,i) \in \{ (1,1), (1,3), (1,4), (2,1) , (2,3) \}$ (for the simplicity of notation we have removed the superscript $N$ from the transmit signals). 

Message $W_k^{(2,b)}$ is mapped to $X_k^{(2,b)}$, where $X_k^{(2,b)}$ is lattice encoded using lattice $\Lambda_k^{(2,b)}$, shift $s_k^{(2,b)}$ and spherical shaping region $S_k^{(2,b)}$, giving a codebook of size $2^{N R_k^{(2)}}$ with power constraint of $P_k^{(2)}$, $k = 1,2$. This codebook is denoted by $(\Lambda_k^{(2,b)} + s_k^{(2,b)}) \cap S_k^{(2,b)}$.

Transmitter $k$ will superimpose all its transmit signals to create $X_k^{(b)}$, its transmit signal during block $b$, \emph{i.e.} $X_1^{(b)} = X_1^{(1,b)} + X_1^{(2,b)} + X_1^{(3,b)} + X_1^{(4,b)}$ and $X_2^{(b)} = X_2^{(1,b)} + X_2^{(2,b)} + X_2^{(3,b)}$.

The power assignments should be such that they are non-negative and satisfy the power constraint at each transmitter, \emph{i.e.}
\begin{equation}
\label{}
\begin{split}
&P_1 = P_1^{(1)} + P_1^{(2)} + P_1^{(3)} \leq 1\\
&P_2 = P_2^{(1)} + P_2^{(2)} \leq 1.
\end{split}
\end{equation}

\noindent  {\bf 2) Feedback Strategy}

Our feedback strategy is motivated through the example in Section~\ref{motivation}. In the example presented in Section~\ref{motivation}, receiver $2$ had to send back the superposition of the codewords corresponding to the cooperative common message of transmitter $1$ and part of its private message to the transmitter $2$ through feedback link. In order to be able to decode the superposition of codewords, we incorporate lattice coding with appropriate power assignment as part of our strategy. 

We set ${\sf SNR} P_1^{(2)} = {\sf INR} P_2^{(2)}$, so that $X_1^{(2,b)}$, and $X_2^{(2,b)}$ arrive at the same power level at receiver $1$ and therefore, $h_{d} X_1^{(2,b)} + h_{c} X_2^{(2,b)}$ is a lattice point. Suppose receiver $1$ is able to decode this lattice index, we refer to it as $I_{\Lambda_{1,2}}^{(b)}$. Then, receiver $1$ sends back $\left( I_{\Lambda_{1,2}}^{(b)} \hspace{1mm} {\mathbf{mod}} \hspace{1mm} 2^{N C_{\sf FB}} \right)$ through the feedback link to transmitter $1$.

Given $\left( I_{\Lambda_{1,2}}^{(b)} \hspace{1mm} {\mathbf{mod}} \hspace{1mm} 2^{N C_{\sf FB}} \right)$, transmitter $1$ removes $h_{d} X_1^{(2,b)}$ and decodes the message index of $W_2^{(2,b)}$. This can be done as long as the total number of lattice points for either of two aligned messages is less than $2^{ N C_{\sf FB}}$, \emph{i.e.} we require $R_1^{(2,b)}, R_2^{(2,b)} \leq C_{\sf FB}$. Since the feedback transmission itself lasts a block, we set $W_1^{(3,b+2)} = W_2^{(2,b)}$.

\noindent  {\bf 3) Decoding}

For simplicity of notation, we ignore the block index and from our description it is clear whether two signals belong to the same block or different ones. We also use the following notation to simplify our equations
\begin{equation}
P_k^{(1:j)} = P_k^{(1)} + P_k^{(2)} + \ldots + P_k^{(j)} \hspace{4mm} k = 1, 2.
\end{equation}

The decoding order of the codewords depends on the channel gains. So, we consider $3$ different scenarios.

\noindent  {\bf 3-a) $\log \left( {\sf INR} \right) \leq \frac{1}{2} \log \left( {\sf SNR} \right)$:}

In this case, we set $R_1^{(4)} = R_2^{(3)} = 0$. In other words, $W_1^{(4)}$ and $W_2^{(3)}$ are deterministic messages. Therefore, the received signal at receiver $1$ is
\begin{equation}
\label{}
Y_1 = h_d \left( X_1^{(1)} + X_1^{(2)} + X_1^{(3)} \right) + h_c \left( X_2^{(1)} + X_2^{(2)} \right) + Z_1.
\end{equation}

At the end of each block, receiver $1$ first decodes $X_1^{(3)}$ by treating all other codewords as noise. $X_1^{(3)}$ can be decoded with small error probability if
\begin{equation}
R_1^{(3)} \leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(3)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(1:2)}} \right).
\end{equation}

It then removes $h_d X_1^{(3)}$ from the received signal and decodes $X_1^{(1)}$ by treating other codewords as noise. $X_1^{(1)}$ is decodable at receiver $1$ with arbitrary small error probability if
\begin{equation}
R_1^{(1)} \leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(1)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(2)} } \right).
\end{equation}

After removing $h_d X_1^{(1)}$, receiver $1$ has access to $h_{d} X_1^{(2)} + h_{c} X_2^{(2)} + h_{c} X_2^{(1)} + Z_1$. Since we have set ${\sf SNR} P_1^{(2)} = {\sf INR} P_2^{(2)}$, $h_{d} X_1^{(2)} + h_{c} X_2^{(2)}$ is a lattice point with some index $I_{\Lambda_{1,2}}^{(b)}$. Receiver $1$ decodes $I_{\Lambda_{1,2}}^{(b)}$ by treating other codewords as noise, and sends back $\left( I_{\Lambda_{1,2}}^{(b)} \hspace{1mm} {\mathbf{mod}} \hspace{1mm} 2^{N C_{\sf FB}} \right)$ to transmitter $1$. From Lemma~\ref{lemma:lattice}, decoding with arbitrary small error probability is feasible if
\begin{equation}
\begin{split}
R_1^{(2)} &\leq \log \left( \frac{ {\sf SNR} P_1^{(2)}}{1 + {\sf INR} P_2^{(1)} } \right)^+\\
R_2^{(2)} &\leq \log \left( \frac{ {\sf INR} P_2^{(2)}}{1 + {\sf INR} P_2^{(1)} } \right)^+,
\end{split}
\end{equation}
we have used the following notation, $\log \left( x \right)^+ = \max \{ \log \left( x \right), 0 \}, \hspace{2mm} x \in \mathbb{R}$.

The decoding at receiver $2$ proceeds as follows. At the end of each block, receiver $2$ removes $h_c X_1^{(3)}$ from its received signal. Note that, $X_1^{(3)}$ is in fact a function of $W_2^{(2,b-2)}$ and hence, it is known to receiver $2$ (assuming successful decoding in the previous blocks). Therefore, the received signal at receiver $2$ after removing $h_c X_1^{(3)}$ is
\begin{equation}
\label{}
Y_2 = h_d \left( X_2^{(1)} + X_2^{(2)} \right) + h_c \left( X_1^{(1)} + X_1^{(2)} \right) + Z_2. 
\end{equation}

Receiver $2$ proceeds by decoding $X_2^{(2)}$ and $X_2^{(1)}$ by treating other codewords as noise. This can be done with arbitrary small error probability if 
\begin{equation}
\begin{split}
R_2^{(2)} &\leq \log \left( \frac{ {\sf SNR} P_2^{(2)}}{1 + {\sf SNR} P_2^{(1)} + {\sf INR} P_1^{(1:2)} } \right)^+ \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_2^{(1)}}{1 + {\sf INR} P_1^{(1:2)} } \right).
\end{split}
\end{equation}

The decoding strategy presented above describes a set of constraints on the rates, which is summerized as follows (loose outer-bounds have been removed).
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(1)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(2)} } \right) \\
R_1^{(2)} &\leq \min \{ \log \left( \frac{ {\sf SNR} P_1^{(2)}}{1 + {\sf INR} P_2^{(1)} } \right)^+, C_{\sf FB} \} \\
R_1^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(3)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(1:2)}} \right) \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_2^{(1)}}{1 + {\sf INR} P_1^{(1:2)} } \right) \\
R_2^{(2)} &\leq \min \{ \log \left( \frac{ {\sf INR} P_2^{(2)}}{1 + {\sf INR} P_2^{(1)} } \right)^+, C_{\sf FB} \}
\end{array} \right.
\end{equation}

Therefore, through the scheme described for this case, we can achieve a sum-rate $R_{\sf SUM}^{(a)} = R_1^{(1)} + R_1^{(2)} + R_2^{(1)} + R_2^{(2)}$, arbitrary close to\footnotemark \footnotetext{Note that $X_1^{(3,b)}$ is a function of the cooperative common message of transmitter $2$, \emph{i.e.} $W_2^{(2,b-2)}$, hence, it does not contain any new information and it is not considered in the sum-rate.}
\begin{align}
\label{eq:rsuma}
R_{\sf SUM}^{(a)} &=  \log \left( 1 + \frac{ {\sf SNR} P_1^{(1)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(2)} } \right) \nonumber \\
&\; + \min \{ \log \left( \frac{ {\sf SNR} P_1^{(2)}}{1 + {\sf INR} P_2^{(1)} } \right)^+, C_{\sf FB} \} \nonumber \\
&\; + \log \left( 1 + \frac{ {\sf SNR} P_2^{(1)}}{1 + {\sf INR} P_1^{(1:2)} } \right) \nonumber \\
&\; + \min \{ \log \left( \frac{ {\sf INR} P_2^{(2)}}{1 + {\sf INR} P_2^{(1)} } \right)^+, C_{\sf FB} \}.
\end{align}

\noindent {\bf 3-b) $\frac{1}{2} \log \left( {\sf SNR} \right) \leq \log \left( {\sf INR} \right) \leq \frac{2}{3} \log \left( {\sf SNR} \right)$:}

The received signal at receiver $1$ in this case, can be written as
\begin{align}
\label{}
Y_1 &= h_d \left( X_1^{(1)} + X_1^{(2)} + X_1^{(3)} + X_1^{(4)} \right) \nonumber \\
&+ h_c \left( X_2^{(1)} + X_2^{(2)} + X_2^{(3)} \right) + Z_1.
\end{align}

At the end of each block, receiver $1$ first decodes $X_1^{(4)}$ by treating all other codewords as noise, and removes $h_d X_1^{(4)}$ from the received signal. At receiver $1$, $X_1^{(4)}$ can be decoded with small error probability if
\begin{equation}
R_1^{(4)} \leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(4)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(1:3)}} \right).
\end{equation}

Next, receiver $1$ decodes $X_1^{(3)}$ by treating other codewords as noise and removes $h_d X_1^{(3)}$ from the received signal. $X_1^{(3)}$ is decodable at receiver $1$ with arbitrary small error probability if
\begin{equation}
R_1^{(3)} \leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(3)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(1:2)} } \right).
\end{equation}

The decoding proceeds by decoding the non-cooperative common message of transmitter $2$, \emph{i.e.} $X_2^{(3)}$ by treating other codewords as noise. $X_2^{(3)}$ can be decoded with arbitrary small error probability if
\begin{equation}
R_2^{(3)} \leq \log \left( 1 + \frac{ {\sf INR} P_2^{(3)}}{1 + {\sf INR} P_2^{(1:2)} + {\sf SNR} P_1^{(1:2)}} \right).
\end{equation}

Receiver $1$ removes $h_c X_2^{(3)}$ from the received signal. It has now access to $h_d X_1^{(2)} + h_c X_2^{(2)} + h_d X_1^{(1)} + h_c X_2^{(1)} + Z_1$. Receiver $1$ decodes the lattice index of $h_d X_1^{(2)} + h_c X_2^{(2)}$, \emph{i.e.} $I_{\Lambda_{1,2}}^{(b)}$, by treating other codewords as noise. It then sends back $\left( I_{\Lambda_{1,2}}^{(b)} \hspace{1mm} {\mathbf{mod}} \hspace{1mm} 2^{N C_{\sf FB}} \right)$ to transmitter $1$. From Lemma~\ref{lemma:lattice}, decoding with arbitrary small error probability is feasible if
\begin{equation}
\begin{split}
R_1^{(2)} &\leq \log \left( \frac{ {\sf SNR} P_1^{(2)}}{1 + {\sf INR} P_2^{(1)} + {\sf SNR} P_1^{(1)} } \right)^+ \\
R_2^{(2)} &\leq \log \left( \frac{ {\sf INR} P_2^{(2)}}{1 + {\sf INR} P_2^{(1)} + {\sf SNR} P_1^{(1)} } \right)^+.
\end{split}
\end{equation}

After decoding and removing $h_{d} X_1^{(2)} + h_{c} X_2^{(2)}$, receiver $1$ decodes $X_1^{(1)}$. This can be done with arbitrary small error probability if
\begin{equation}
R_1^{(1)} \leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(1)}}{1 + {\sf INR} P_2^{(1)} } \right).
\end{equation}

Similar to the previous case, receiver $2$ removes $X_1^{(3)}$ from its received signal. The decoding at receiver $2$ proceeds as follows. Receiver $2$ decodes $X_2^{(3)}$ by treating other codewords as noise and removes $h_d X_2^{(3)}$ from the received signal. Next, $X_2^{(2)}$, the non-cooperative common message of transmitter $1$, will be decoded by treating other codewords as noise. Receiver $2$ removes $h_d X_2^{(2)}$ from the received signal and then, decodes $X_1^{(4)}$ by treating other codewords as noise. After removing $h_c X_1^{(4)}$, the private message of transmitter $2$, \emph{i.e.} $X_2^{(1)}$ will be decoded. The decoding can be performed with arbitrary small error probability if 
\begin{equation}
\begin{split}
R_2^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_2^{(3)}}{1 + {\sf SNR} P_2^{(1:2)} + {\sf INR} ( P_1 - P_1^{(3)} ) } \right) \\
R_2^{(2)} &\leq \log \left( \frac{ {\sf SNR} P_2^{(2)}}{1 + {\sf SNR} P_2^{(1)} + {\sf INR} ( P_1 - P_1^{(3)} ) } \right)^+ \\
R_1^{(4)} &\leq \log \left( 1 + \frac{ {\sf INR} P_1^{(4)}}{1 + {\sf INR} P_1^{(1:2)} + {\sf SNR} P_2^{(1)}} \right) \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_2^{(1)}}{1 + {\sf INR} P_1^{(1:2)} } \right) 
\end{split}
\end{equation}

The decoding strategy presented above describes a set of constraints on the rates, which is summerized as follows (loose upper-bounds have been eliminated).
\begin{equation}
\label{}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(1)}}{1 + {\sf INR} P_2^{(1)} } \right) \\
R_1^{(2)} &\leq \min \{ \log \left( \frac{ {\sf SNR} P_1^{(2)}}{1 + {\sf INR} P_2^{(1)} + {\sf SNR} P_1^{(1)} } \right)^+, C_{\sf FB} \} \\
R_1^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_1^{(3)}}{1 + {\sf INR} P_2 + {\sf SNR} P_1^{(1:2)} } \right) \\
R_1^{(4)} &\leq \log \left( 1 + \frac{ {\sf INR} P_1^{(4)}}{1 + {\sf INR} P_1^{(1:2)} + {\sf SNR} P_2^{(1)}} \right) \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR} P_2^{(1)}}{1 + {\sf INR} P_1^{(1:2)} } \right) \\
R_2^{(2)} &\leq \min \{ \log \left( \frac{ {\sf INR} P_2^{(2)}}{1 + {\sf INR} P_2^{(1)} + {\sf SNR} P_1^{(1)} } \right)^+, C_{\sf FB} \} \\
R_2^{(3)} &\leq \log \left( 1 + \frac{ {\sf INR} P_2^{(3)}}{1 + {\sf INR} P_2^{(1:2)} + {\sf SNR} P_1^{(1:2)} } \right)
\end{array} \right.
\end{equation}

Therefore, through the achievability scheme described above, we can achieve a sum-rate $R_{\sf SUM}^{(b)} = R_1^{(1)} + R_1^{(2)} + R_1^{(4)} + R_2^{(1)} + R_2^{(2)} + R_2^{(3)}$, arbitrary close to\footnotemark \footnotetext{Note that $X_1^{(3,b)}$ is a function of the cooperative common message of transmitter $2$, \emph{i.e.} $W_2^{(2,b-2)}$, hence it is not considered in the sum-rate.}
\begin{align}
\label{eq:rsumb}
R_{\sf SUM}^{(b)} &=  \log \left( 1 + \frac{ {\sf SNR} P_1^{(1)}}{1 + {\sf INR} P_2^{(1)} } \right) \nonumber \\
&+ \min \{ \log \left( \frac{ {\sf SNR} P_1^{(2)}}{1 + {\sf INR} P_2^{(1)} + {\sf SNR} P_1^{(1)} } \right)^+, C_{\sf FB} \} \nonumber \\
&+ \log \left( 1 + \frac{ {\sf INR} P_1^{(4)}}{1 + {\sf INR} P_1^{(1:2)} + {\sf SNR} P_2^{(1)}} \right) \nonumber \\
&+ \log \left( 1 + \frac{ {\sf SNR} P_2^{(1)}}{1 + {\sf INR} P_1^{(1:2)} } \right) \nonumber \\
&+ \min \{ \log \left( \frac{ {\sf INR} P_2^{(2)}}{1 + {\sf INR} P_2^{(1)} + {\sf SNR} P_1^{(1)} } \right)^+, C_{\sf FB} \} \nonumber \\
&+ \log \left( 1 + \frac{ {\sf INR} P_2^{(3)}}{1 + {\sf INR} P_2^{(1:2)} + {\sf SNR} P_1^{(1:2)} } \right).
\end{align}

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%

\noindent {\bf 3-c) $2 \log \left( {\sf SNR} \right) \leq \log \left( {\sf INR} \right)$: }

In this case there is no need to decode superposition of messages and as a reslut, the scheme becomes simpler. Set $R_1^{(1)}, R_1^{(2)}$ and $R_2^{(1)}$ equal to zero. In other words, $W_1^{(1)}, W_1^{(2)}$ and $W_2^{(1)}$ are deterministic messages. Hence the received signal at receiver $1$ is
\begin{equation}
\label{}
Y_1 = h_d \left( X_1^{(3)} + X_1^{(4)} \right) + h_c \left( X_2^{(2)} + X_2^{(3)} \right) + Z_1,
\end{equation}
and at receiver $2$, we have
\begin{equation}
\label{}
Y_2 = h_d \left( X_2^{(2)} + X_2^{(3)} \right) + h_c \left( X_1^{(3)} + X_1^{(4)} \right) + Z_2.
\end{equation}

As for the feedback strategy, receiver $1$ decodes $X_2^{(2)}$ by treating other codewords as noise, and sends the lattice index of $W_2^{(2)}$ back to transmitter $1$ during the following block. Transmitter $1$ later encodes this message as $X_1^{(3)}$ and transmits it. It is worth mentioning that in this case, it is in fact receiver $2$ who wants to exploit the feedback link of user $1$ to get part of its message. In other words, we have two paths for information flow from transmitter $2$ to receiver $2$; one through the direct link between them and the other one through receiver $1$, feedback link and transmitter $1$. The decoding works very similar to what we described above and we get the following set of constraints to guarantee small error probability at the decoders.
\begin{equation}
\label{ach1}
\left\{ \begin{array}{ll}
R_1^{(3)} &\leq \log \left( 1 + \frac{{\sf INR} P_1^{(3)}}{1+{\sf SNR} P_2} \right) \\
R_1^{(4)} &\leq \log \left( 1 + \frac{{\sf SNR} P_1^{(4)}}{1+{\sf SNR} P_1^{(3)}} \right) \\
R_2^{(2)} &\leq \min \{ \log \left( \frac{{\sf INR} P_2^{(2)}}{1+{\sf SNR} P_1} \right)^+, C_{\sf FB} \} \\
R_2^{(3)} &\leq \log \left( 1 + \frac{{\sf SNR} P_2^{(3)}}{1+{\sf SNR} P_2^{(2)}} \right)
\end{array} \right.
\end{equation}

As before $X_1^{(3,b)}$ is a function of $W_2^{(2,b-2)}$. Therefore, we can achieve a sum-rate $R_{\sf SUM}^{(c)} = R_1^{(4)} + R_2^{(2)} + R_2^{(3)}$, arbitrary close to
\begin{align}
\label{eq:rsumc}
R_{\sf SUM}^{(c)} &= \log \left( 1 + \frac{{\sf SNR} P_1^{(4)}}{1+{\sf SNR} P_1^{(3)}} \right) \nonumber \\
&+ \min \{ \log \left( \frac{{\sf INR} P_2^{(2)}}{1+{\sf SNR} P_1} \right)^+, C_{\sf FB} \} \nonumber \\
&\; \quad \log \left( 1 + \frac{{\sf SNR} P_2^{(3)}}{1+{\sf SNR} P_2^{(2)}} \right).
\end{align}

\noindent {\bf General Feedback Assignment}

In the rest of this subsection, we describe our achievability scheme for general feedback capacity assignment based on a combination of the achievability schemes for the extreme cases. Let $C_{\sf FB1} = \lambda C_{\sf FB}$ and $C_{\sf FB2} = \left( 1 - \lambda \right) C_{\sf FB}$, such that $0 \leq \lambda \leq 1$. We call the achievable sum-rate of the extreme case $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$ by $R_{\sf SUM}^{C_{\sf FB2} = 0}$, and similarly, we refer to the achievable sum-rate of the other extreme case by $R_{\sf SUM}^{C_{\sf FB1} = 0}$.
%Note that since we consider symmetric channel gains, the achievable sum-rate is the same for the extreme cases, we refer to it as $\mathcal{R}^\ast$.

\begin{figure}[ht]
\centering
\includegraphics[width=8cm]{feedbackassignment1.pdf}
\caption{Achievability strategy for $C_{\sf FB1} = \lambda C_{\sf FB}$ and $C_{\sf FB2} = \left( 1 - \lambda \right) C_{\sf FB}$.}
\label{feedback12}
\end{figure}

We split any block $b$, $b = 1,2,\ldots,B-2$, of length $N$ into two sub-blocks: $b_1$ of length $\lambda N$ and $b_2$ of length $\left( 1 - \lambda \right) N$, see Figure~\ref{feedback12} for a depiction. Then, our achievability scheme is as follows. During $b_1$, we implement the transmission strategy of the extreme case $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$, with a block length of $\lambda N$; and during $b_2$, the achievability scheme of the extreme case $C_{\sf FB1} = 0$ and $C_{\sf FB2} = C_{\sf FB}$, with a block length of $\left( 1 - \lambda \right) N$.

At the end of each sub-block, receivers decode the messages as described before and create the feedback messages. During block $b+1$ the feedback messages of sub-blocks $b_1$ and $b_2$ will be sent back to corresponding transmitters, as shown in Figure~\ref{feedback12}. Note that we use $C_{\sf FB1}$ during the entire length of block $b+1$, hence the effective feedback rate of user $1$ (total feedback use divided by number of transmission time slots), would be
\begin{equation}
C_{\sf FB1}^{\sf eff} = \frac{N C_{\sf FB1}}{\lambda N} = \frac{\lambda N C_{\sf FB}}{\lambda N} = C_{\sf FB}
\end{equation}

Hence, we can implement the achievability strategy corresponding to the extreme case $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$. Similar argument is valid for the other extreme case. With this achievability scheme, as $N$ goes to infinity, we achieve a sum-rate of $\lambda R_{\sf SUM}^{C_{\sf FB2} = 0} + \left( 1 - \lambda \right) R_{\sf SUM}^{C_{\sf FB1} = 0}$.

==> gaussian.tex <==
In this section, we consider the symmetric two-user Gaussian IC with rate-limited feedback. The Gaussian model is described in section~\ref{problem}. For the symmetric two-user Gaussian IC, we assume:
\begin{equation}
\begin{split}
& {\sf SNR} = {\sf SNR}_1 = {\sf SNR}_2 \\
& {\sf INR} = {\sf INR}_{12} = {\sf INR}_{21} 
\end{split}
\end{equation}

As mentioned before, we focus on the sum-rate capacity of this network and we characterize it to within a constant number of bits independent of all channel parameters. The following theorem describes our main contribution under Gaussian model.

\begin{theorem} \label{THM:Gaussian-sumrate}
The sum-rate capacity of the two-user Gaussian IC with rate-limited feedback is included in the set $\bar{\mathcal{C}}$ of $(R_1,R_2)$ such that
\begin{align}
\label{eq:sum1}
R_1 + R_2 &\leq \log \left( 1 +  (1- \rho^2) \mathsf{SNR}_1 \right) \nonumber \\
&+ \log \left( 1 +  (1- \rho^2) \mathsf{SNR}_2 \right) + C_{\sf FB1 } + C_{\sf FB2 } \\
\label{eq:sum2}
R_1 + R_2 &\leq \log \left( 1 +  \frac{ (1- \rho^2) \mathsf{SNR}_1}{ 1 + (1- \rho^2) \mathsf{INR}_{12}} \right) \nonumber \\
&+  \log \left( 1+ \mathsf{SNR}_2  + \mathsf{INR}_{12} + 2 \rho \sqrt{ \mathsf{SNR}_2  \cdot \mathsf{INR}_{12}} \right) \\
\label{eq:sum3}
R_1 + R_2 &\leq \log \left( 1 +  \frac{ (1- \rho^2) \mathsf{SNR}_2}{ 1 + (1- \rho^2) \mathsf{INR}_{21}} \right) \nonumber \\
& +  \log \left( 1+ \mathsf{SNR}_1  + \mathsf{INR}_{21} + 2 \rho \sqrt{ \mathsf{SNR}_1  \cdot \mathsf{INR}_{21}} \right) \\
\label{eq:sum4}
R_1 + R_2 & \leq \log \left( 1 + (1- \rho^2)  {\sf INR}_{21} + \frac{ (1- \rho^2){\sf SNR}_1 }{1+ (1- \rho^2) {\sf INR}_{12}} \right) \nonumber \\
&\; + \log \left( 1 + (1- \rho^2)  {\sf INR}_{12} + \frac{ (1- \rho^2){\sf SNR}_2 }{1+ (1- \rho^2) {\sf INR}_{21}} \right) \nonumber \\
&\; + \min \left \{ C_{\sf FB1}, \log \left( 1 +  (1- \rho^2) \mathsf{INR}_{21} \right) \right \} \nonumber \\
&\; + \min \left \{ C_{\sf FB2}, \log \left( 1 +  (1- \rho^2) \mathsf{INR}_{12} \right) \right \}
\end{align}
\end{theorem}

In Appendix~\ref{Appendix:Gaussian}, we present an outer-bound on the capacity region of the two-user Gaussian interference channel with rate-limited feedback in Theorem~\ref{theorem:Gaussianouterbound}. The converse for Theorem~\ref{THM:Gaussian-sumrate} is then a direct result of Theorem~\ref{theorem:Gaussianouterbound}. The rest of this section is dedicated to describing the achievability scheme. %Table~\ref{table:Gaussian} is the Gaussian counterpart of Table~\ref{table:linear}.

%We considered our problem under linear deterministic model in Section~\ref{linear} and we extracted the cases where feedback increases the sum-rate capacity. As we can see in Table~\ref{table:linear} for the linear deterministic case, there are cases where feedback cannot provide us with any gain in terms of achievable sum-rate. In those cases under linear deterministic or Gaussian model, we simply use the achievability scheme presented in~\cite{Etkin} for the non-feedback case. As a result, we mainly focus on cases where having feedback in the network helps us increase the sum-rate capacity compared to non-feedback case. %Therefore, for any case that we do not provide an achievability scheme, one can use the results developed in~\cite{Etkin} for the non-feedback scenario.
%We first translate Table~\ref{table:linear} to Gaussian model, \emph{i.e.} Table~\ref{table:Gaussian}. Then, we will describe our achievability strategy in a case by case manner. Table~\ref{table:Gaussian} is the Gaussian counterpart of Table~\ref{table:linear}.

\begin{theorem} \label{THM:Gaussian-sumrate-ach}
The sum-rate capacity of the two-user Gaussian IC with rate-limited feedback includes the set $\mathcal{R}$ of $(R_1,R_2)$ such that
\begin{align}
\label{eq:sum1}
R_1 + R_2 &\leq \log \left( 1 +  (1- \rho^2) \mathsf{SNR}_1 \right) \nonumber \\
&+ \log \left( 1 +  (1- \rho^2) \mathsf{SNR}_2 \right) + C_{\sf FB1 } + C_{\sf FB2 } \\
\label{eq:sum2}
R_1 + R_2 &\leq \log \left( 1 +  \frac{ (1- \rho^2) \mathsf{SNR}_1}{ 1 + (1- \rho^2) \mathsf{INR}_{12}} \right) \nonumber \\
&+  \log \left( 1+ \mathsf{SNR}_2  + \mathsf{INR}_{12} + 2 \rho \sqrt{ \mathsf{SNR}_2  \cdot \mathsf{INR}_{12}} \right) \\
\label{eq:sum3}
R_1 + R_2 &\leq \log \left( 1 +  \frac{ (1- \rho^2) \mathsf{SNR}_2}{ 1 + (1- \rho^2) \mathsf{INR}_{21}} \right) \nonumber \\
& +  \log \left( 1+ \mathsf{SNR}_1  + \mathsf{INR}_{21} + 2 \rho \sqrt{ \mathsf{SNR}_1  \cdot \mathsf{INR}_{21}} \right) \\
\label{eq:sum4}
R_1 + R_2 & \leq \log \left( 1 + (1- \rho^2)  {\sf INR}_{21} + \frac{ (1- \rho^2){\sf SNR}_1 }{1+ (1- \rho^2) {\sf INR}_{12}} \right) \nonumber \\
&\; + \log \left( 1 + (1- \rho^2)  {\sf INR}_{12} + \frac{ (1- \rho^2){\sf SNR}_2 }{1+ (1- \rho^2) {\sf INR}_{21}} \right) \nonumber \\
&\; + \min \left \{ C_{\sf FB1}, \log \left( 1 +  (1- \rho^2) \mathsf{INR}_{21} \right) \right \} \nonumber \\
&\; + \min \left \{ C_{\sf FB2}, \log \left( 1 +  (1- \rho^2) \mathsf{INR}_{12} \right) \right \}
\end{align}
\end{theorem}

We first provide a brief outline of the proof. Our achievability scheme is a based on Block Markov coding, where we use backward decoding at the receivers. The scheme is implemented over $B$ blocks. In each block (with the exception of the last two), new messages are transmitted. At the end of a block, each receiver creates a feedback message according to our feedback strategy and sends it back to its corresponding transmitter. This will provide each transmitter with part (or all) of the interference from the other user. Each transmitter encodes this interfering message and transmit it to its receiver during a different block. Through this part of the transmit signal, receivers will be able to complete the decoding of the messages received previously.

As we have seen in Section~\ref{motivation}, each receivers may need to decode the superposition of the cooperative common message of the other transmitter and part of the private message of its corresponding transmitter. In order to be able to decode the superposition of messages in Gaussian model, we use lattice codes as it will be discussed later (note that not all messages will be encoded as lattice points).

%One of the main challenges when dealing with rate-limited feedback, is to precisely determine what to be sent back through feedback links. This was not an issue for the authors of~\cite{Suh}, since they considered infinite feedback capacity and therefore, the whole output at a receiver could be provided to its intended transmitter with some delay. However, this is not possible with rate-limited feedback.

%To efficiently overcome this issue, we use lattice codes. In Section~\ref{motivation}, we saw that a receiver (who needs to create a feedback message) sends back the \emph{superposition} of some messages to its corresponding transmitter under the deterministic model. To implement this idea in Gaussian IC, we incorporate lattice coding in our scheme. The reason is that by appropriate power assignment, interfering messages encoded as lattice points create a new lattice point and hence, lattice coding is a suitable option for our feedback strategy. We provide a brief overview of lattice coding in the following subsection. 

\subsection{Lattice Coding Preliminaries}

In this subsection, we briefly go over some preliminaries on lattice coding and summerize the results that are going to be used in this paper. %A lattice $\Lambda$ of dimension $n$ is described by
%\begin{equation}
%\Lambda = \{ \lambda = \mathbf{G}x : x \in \mathbb{Z}^n \},
%\end{equation}
%where $G$ is the generator matrix that describes the lattice. Denote the fundamental Voronoi region of lattice $\Lambda$ by $\Omega_\Lambda$ and the volume of $\Omega_\Lambda$ by $V_\Lambda$. We use lattices using construction A in \cite{lattice}. as described below.
A lattice is a discrete additive subgroup of $\mathbb{R}^n$. The fundamental volume $V_f(\Lambda)$ of a lattice $\Lambda$ is the reciprocal of the number of lattice points per unit volume.

Given integer $p$, denote the set of integers modulo $p$ by $\mathbb{Z}_p$. Let $\mathbb{Z}^n \rightarrow \mathbb{Z}_p^n: v \mapsto \bar{v}$ be the componentwise modulo $p$ operation over integer vectors. Also, let $C$ denote a linear $(n,k)$ code over $\mathbb{Z}_p$. Then the lattice $\Lambda_C$ defined as
\begin{equation}
\Lambda_C = \{ v \in \mathbb{Z}^n : \bar{v} \in C \},
\end{equation}
is generated with respect to the linear code $C$ (see \cite{lattice} for details). In \cite{lattice}, it has been shown that there exists good lattice codes for communication channels, \emph{i.e.} codes that achieve a rate close to the capacity of the channel with arbitrary small decoding error probability. We summerize that result here.

Consider a point-to-point communication scenario over an additive noise channel
\begin{equation}
\label{eq:p2p}
Y = X + Z
\end{equation}
where $X$ is the transmitted signal with power constraint $P$, $Y$ is the received signal and $Z$ is the additive noise process with zero mean and variance $\sigma^2$.

Set $\mathcal{B}$ of linear codes over $\mathbb{Z}_p$ is called balanced if every nonzero element of $\mathbb{Z}_p^n$ is contained in the same number of codes in $\mathcal{B}$. Define $\mathcal{L}_\mathcal{B}$ as
\begin{equation}
\label{eq:L}
\mathcal{L}_\mathcal{B} = \{ \Lambda_C : C \in \mathcal{B} \}.
\end{equation}
based on the aforementioned definitions, we have the following result for lattice coding.

%Consider a point to point communication scenario over an additive noise channel
%\begin{equation}
%\label{eq:p2p}
%Y = X + Z
%\end{equation}
%where $X$ is the transmitted signal, $Y$ is the received signal and $Z$ is the additive noise process with zero mean and variance $\sigma^2$. We have the following result for lattice coding.

\begin{lemma}[\cite{lattice}]
Consider a single user point-to-point additive noise channel described in (\ref{eq:p2p}). Let $\mathcal{B}$ be a balanced set of linear $(n, k)$ codes over $\mathbb{Z}_p$. Averaged over all lattices from the set $\mathcal{L}_\mathcal{B}$ defined in (\ref{eq:L}), each scaled by $\gamma > 0$ and with a fundamental volume $V$, we have that for any $\delta > 0$, the
average probability of decoding error is bounded by
\begin{equation}
\label{}
\bar{P}_e < (1+\delta) \frac{n\frac{1}{2}\log \left( 2 \pi e \sigma^2 \right)}{V}
\end{equation}
for sufficiently large $p$ and small $\gamma$ such that $\gamma^n p^{n-k} = V$. %Hence, the probability of decoding error for at least three fourths of the lattices in $\mathcal{L}_\mathcal{B}$ satisfies
%\begin{equation}
%\label{}
%P_e < 4 (1+\delta) \frac{n\frac{1}{2}\log \left( 2 \pi e \sigma^2 \right)}{V}.
%\end{equation}
\end{lemma}

Proof can be found in \cite{lattice}. The next lemma describes the existence of a good lattice code for a single user AWGN channel.

\begin{lemma}[\cite{lattice}]
\label{lemma:lattice}
Consider a point-to-point additive noise channel described in (\ref{eq:p2p}) such that the transmitter satisfies a power constraint of $P$. Then, we can choose a lattice $\Lambda$ generated using construction A, a shift $s$\footnotemark \footnotetext{shift $s$ is a vector in $\mathbb{R}^n$ and it is required in order to prove of existence of good lattice codes, see \cite{lattice} for more details.} and a shaping region $S$\footnotemark \footnotetext{We need to consider the intersection of a lattice with some shaping region $S \subset \mathbb{R}^n$ to satisfy the power constraint.} such that the codebook $(\Lambda + s) \cap S$ achieves a rate $R$ with arbitrarily small probability of error if
\begin{equation}
\label{}
R \leq \frac{1}{2} \log \left( \frac{P}{\sigma^2} \right)
\end{equation}
\end{lemma}

In other words, Lemma~\ref{lemma:lattice} describes the existence of a lattice code with sufficient codewords. Proof can be found in \cite{lattice}. 

\begin{remark}
In this paper, we consider complex AWGN channels. Similar to Lemma~\ref{lemma:lattice}, one can show that using lattice codes, a rate of $\log \left( \frac{P}{\sigma^2} \right)$ is achievable in a complex AWGN channel.
\end{remark}

\subsection{Acievability Strategy}

In this subsection, we describe our achievability scheme for Theorem~\ref{THM:Gaussian-sumrate}. This achievability scheme is general in the sense that it is based on some adjustable parameters, \emph{i.e.} power levels. We first present our scheme without specifying the values of these parameters and in Section~\ref{gap}, we present our choice of these parameters and we analyze the performance of the strategy. 

%We first esablish the achievability scheme in its most general form, \emph{i.e.} weak interference regime, and we then show how it can be adjusted to work for a different regime, namely strong interference regime.

%In this subsection, we present our achievability strategy for case $2$ and we assume $B^\prime_4$ is the effective outer bound and we have
%\begin{align}
%\left( \frac{ {\sf SNR}_1 }{1+ {\sf INR}_{12}} \right)  \leq \left( 1 + {\sf INR}_{21} \right) \hspace{4mm} \text{and} \hspace{4mm} \left( \frac{ {\sf SNR}_2 }{1+ {\sf INR}_{21}} \right)  \leq \left( 1 + {\sf INR}_{12} \right).
%\end{align}

It is sufficient to consider only the extreme case where $C_{\sf FB1} = C_{\sf FB}$ and $C_{\sf FB2} = 0$. The achievability scheme for the other extreme case, \emph{i.e.} $C_{\sf FB1} = 0$ and $C_{\sf FB2} = C_{\sf FB}$, is very similar and is therefore omitted. Later in Section~\ref{gap}, we will show that for any other feedback configuration a time sharing of the two achievability schemes provides us with the desired result.

{\bf Achievability Strategy 1:}

{\bf 1) Codebook Generation and Encoding}

In block $b$, $b = 1,2,\ldots,B-2$, transmitter $1$ has $4$ independent messages $W_1^{(1,b)}, W_1^{(2,b)}, W_1^{(3,b)}$ and $W_1^{(4,b)}$ for receiver $1$, where $W_1^{(i,b)} \in \{ 1, 2, \ldots, 2^{N R_1^{(i)}} \}$. Out of these four messges $W_1^{(1,b)}, W_1^{(2,b)}$ and $W_1^{(4,b)}$ are new messages. We further describe $W_1^{(3,b)}$ when we describe the feedback strategy. On the other hand, transmitter $2$ has $3$ new independent messages $W_2^{(1,b)}, W_2^{(2,b)}$ and $W_2^{(3,b)}$ for receiver $2$.%The message splitting is inspired by our achievability strategy for the deterministic model, \emph{i.e.} at each transmitter we can distinguish $3$ different categories of messages: (1) cooperative common message, (2) non-cooperative common message, and (3) private message (see Secion~\ref{motivation} for more details).

%The private message is only decodable at the intended receiver and it arrives at noise level at the unintended receiver. Here, messages $W_1^{(1,b)}$ and $W_1^{(2,b)}$ form the private message of transmitter $1$. It will be later clarified why we split the private message into two parts. The non-cooperative common message is visible to both receivers, however it is not required to be sent back as part of the feedback message at either receivers. In this case, $W_1^{(4,b)}$ is the non-cooperative common message of transmitter $1$. With the specific assumptions on channel gains, there is no cooperative common message at transmitter $1$ in this case.

%Transmitter $2$ during any block $b$, will transmit $3$ new independent messages $W_2^{(1,b)}, W_2^{(2,b)}$ and $W_2^{(3,b)}$ to receiver $2$. Here, $W_2^{(1,b)}$ is the private message of transmitter $2$, while $W_2^{(2,b)}$ and $W_2^{(3,b)}$ are the cooperative and non-cooperative common messages of transmitter $2$ respectively. Similar to transmitter $1$, transmitter $2$ creates $X_2^{(b)} = X_2^{(1,b)} + X_2^{(2,b)} + X_2^{(3,b)}$.

At transmitter $k$, message $W_k^{(i,b)}$ is mapped to $X_k^{(i,b)}$, where $X_k^{(i,b)}$ is a Gaussian codeword pricked from a codebook of size $2^{N R_k^{(i)}}$ and any elemnet of this codebook is distributed as i.i.d. $\mathcal{CN}(0,P_k^{(i)})$, $(k,i) = \{ (1,3) , (1,4), (2,1) , (2,3) \}$ (for the simplicity of notation we have removed the superscript $N$ from the transmit signals). 

However, message $W_k^{(i,b)}$ is mapped to $X_k^{(i,b)}$, where $X_k^{(i,b)}$ is lattice encoded using lattice $\Lambda_k^{(i,b)}$, shift $s_k^{(i,b)}$ and spherical shaping region $S_k^{(i,b)}$, giving a codebook of size $2^{N R_k^{(i)}}$ with power constraint of $P_k^{(i)}$, $(k,i) = (1,1),(1,2),(2,2)$. This codebook is denoted by $(\Lambda_k^{(i,b)} + s_k^{(i,b)}) \cap S_k^{(i,b)}$. Transmitter $k$ will superimpose all its transmit signals to create $X_k^{(b)}$, \emph{i.e.} $X_1^{(b)} = X_1^{(1,b)} + X_1^{(2,b)} + X_1^{(3,b)} + X_1^{(4,b)}$ and $X_2^{(b)} = X_2^{(1,b)} + X_2^{(2,b)} + X_2^{(3,b)}$.

The power assignments should be such that they satisfy the power constraint at each transmitter, \emph{i.e.}
\begin{equation}
\label{powerconstraints1a}
\begin{split}
&P_1 = P_1^{(1)} + P_1^{(2)} + P_1^{(3)} + P_1^{(4)} \leq 1\\
&P_2 = P_2^{(1)} + P_2^{(2)} + P_2^{(3)} \leq 1.
\end{split}
\end{equation}

{\bf 2) Feedback Strategy}

Our feedback strategy is motivated through the example in Section~\ref{motivation}. There are cases such as the one presented in Section~\ref{motivation} where a receiver $2$ had to send back the superposition of the cooperative common message of transmitter $1$ and part of its private message to the transmitter $2$ through feedback link. %(the fact that part of the private message will be sent back to transmitter, justifies splitting the private message of transmitter $1$ into two parts). 
In order to be able to decode the superposition of messages, we incorporate lattice coding with appropriate power assignment as part of our strategy. %Through this scheme receivers (if required to do so) will be able to decode the superposition of the cooperative common message of the interfering transmitter and part of the private message from the intended transmitter. 

We either set ${\sf SNR_1} P_1^{(1)} = {\sf INR_{21}} P_2^{(2)}$ or ${\sf SNR_1} P_1^{(2)} = {\sf INR_{21}} P_2^{(2)}$, so that either of $X_1^{(1,b)}$ or $X_1^{(2,b)}$, and $X_2^{(2,b)}$ arrive at the same power level at receiver $1$ and therefore, $h_{11} X_1^{(1,b)} + h_{21} X_2^{(2,b)}$ or $h_{11} X_1^{(2,b)} + h_{21} X_2^{(2,b)}$ is a lattice point. Suppose receiver $1$ is able to decode this lattice index, we refer to it as $I_{\Lambda_{1,2}}^{(b)}$. Then, receiver $1$ sends back $\left( I_{\Lambda_{1,2}}^{(b)} \hspace{1mm} {\mathbf{mod}} \hspace{1mm} 2^{N C_{\sf FB}} \right)$ through the feedback link to transmitter $1$.

Given $\left( I_{\Lambda_{1,2}}^{(b)} \hspace{1mm} {\mathbf{mod}} \hspace{1mm} 2^{N C_{\sf FB}} \right)$, transmitter $1$ removes $h_{11} X_1^{(1)}$ or $h_{11} X_1^{(2)}$ and decodes the message index of $W_2^{(2,b)}$. This can be done as long as the total number of lattice points for either of two aligned messages is less than $2^{ N C_{\sf FB}}$, \emph{i.e.} we require $R_1^{(2,b)}, R_2^{(2)} \leq C_{\sf FB}$. Since the feedback transmission itself lasts a block, we set $W_1^{(3,b+2)} = W_2^{(2,b)}$.

{\bf 3) Decoding}

For simplicity of notation, we ignore the block index and from our description it is clear whether two signals belong to the same block or different ones. At the end of any block, receiver $1$ first decodes $X_1^{(4)}$ and removes it from the received signal. Next, receiver $1$ decodes $X_1^{(3)}$ and removes it from the received signal (at the end of first and second block, there is no $X_1{(3)}$ to decode). The decoding proceeds by decoding the non-cooperative common message of transmitter $2$, \emph{i.e.} $X_2^{(3)}$. After removing $X_2^{(3)}$, receiver $1$ faces two scenarios: it either decodes the \emph{superposition} of $X_2^{(2)}$, the cooperative common message of transmitter $2$, and $X_1^{(2)}$ and then decodes $X_1^{(1)}$, or it decodes $X_1^{(2)}$ and then decodes the superposition of $X_1^{(1)}$ and $X_2^{(2)}$.

The decoding proceeds as follows at receiver $2$. At the end of any block $b$, receiver $2$ removes $X_1^{(3)}$ from its received signal before decoding any messages (at the end of first and second block, there is no $X_1{(3)}$ to decode). Note that, $X_1^{(3)}$ is in fact repetition of $W_2^{(2,b-2)}$ and hence, it is known to receiver $2$. Receiver $2$ starts by decoding $X_2^{(3)}$ and removes it from the received signal. Next, $X_2^{(2)}$ and $X_1^{(4)}$, the non-cooperative common message of transmitter $1$, will be decoded. Finally, the private message of transmitter $2$, \emph{i.e.} $X_2^{(1)}$ will be decoded.

We derive a set of inequalities to assure arbitrary small error probability at the decoders. We use the following notation to simplify our equations:
\begin{equation}
P_k^{(1:j)} = P_k^{(1)} + P_k^{(2)} + \ldots + P_k^{(j)} \hspace{4mm} k = 1, 2.
\end{equation}

At receiver $1$, $W_1^{(4)}$ can be decoded with small error probability treating other signals as noise if
\begin{equation}
R_1^{(4)} \leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(4)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} P_1^{(1:3)}} \right).
\end{equation}

As described before, receiver $1$ removes $X_1^{(4)}$ from the received signal. $W_1^{(3)}$ is decodable at receiver $1$ with arbitrary small error probability if
\begin{equation}
R_1^{(3)} \leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(3)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} P_1^{(1:2)} } \right).
\end{equation}

At this point, receiver $1$ should be able to decode $W_2^{(3)}$ treating other signals as noise. Decoding $W_2^{(3)}$ with arbitrary small error probability requires
\begin{equation}
R_2^{(3)} \leq \log \left( 1 + \frac{ {\sf INR_{21}} P_2^{(3)}}{1 + {\sf INR_{21}} P_2^{(1:2)} + {\sf SNR_1} P_1^{(1:2)}} \right).
\end{equation}

Receiver $1$ removes $X_2^{(3)}$ and has now access to $h_{11} X_1^{(2)}$ interfered by $h_{21} X_2^{(2)}$. As we described the feedback strategy, receiver $1$ decodes $I_{\Lambda_{1,2}}^{(b)}$ and send back $\left( I_{\Lambda_{1,2}}^{(b)} \hspace{1mm} {\mathbf{mod}} \hspace{1mm} 2^{N C_{\sf FB}} \right)$ to transmitter $1$. From Lemma~\ref{lemma:lattice} and the fact that we set ${\sf SNR_1} P_1^{(2)} = {\sf INR_{21}} P_2^{(2)}$, decoding with arbitrary small error probability is feasible if
\begin{equation}
\begin{split}
R_1^{(2)} &\leq \log \left( \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)} + {\sf SNR_1} P_1^{(1)} } \right)\\
R_2^{(2)} &\leq \log \left( \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)} + {\sf SNR_1} P_1^{(1)} } \right).
\end{split}
\end{equation}

After decoding and removing $h_{11} X_1^{(2)} + h_{21} X_2^{(2)}$, receiver $1$ decodes $W_1^{(1)}$. This can be done with arbitrary small error probability if
\begin{equation}
R_1^{(1)} \leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} P_2^{(1)} } \right).
\end{equation}

Receiver $2$ first removes $W_1^{(3)}$ from its received signal as described before. Decoding with arbitrary small error probability at receiver $2$ is guaranteed if
\begin{equation}
\begin{split}
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} P_1^{(1:2)} } \right) \\
R_1^{(4)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(4)}}{1 + {\sf INR_{12}} P_1^{(1:2)} + {\sf SNR_2} P_2^{(1)}} \right) \\
R_2^{(2)} &\leq \log \left( \frac{ {\sf SNR_2} P_2^{(2)}}{1 + {\sf SNR_2} P_2^{(1)} + {\sf INR_{12}} ( P_1 - P_1^{(3)} ) } \right) \\
R_2^{(3)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(3)}}{1 + {\sf SNR_2} P_2^{(1:2)} + {\sf INR_{12}} ( P_1 - P_1^{(3)} ) } \right).
\end{split}
\end{equation}

%We will now describe our feedback strategy in more details. At the beginning of any other block $b$ (with the exception of first two ones), transmitter $1$ will receive a lattice index through the feedback link from which it can decode the cooperative common message of transmitter $2$ transmitted two blocks ago, \emph{i.e.} $W_2^{(2,b-2)}$. This message will encoded as $X_1^{(3,b)}$. Since this message is already known to receiver $2$, \emph{i.e.} it has been already decoded at the end of block $b-2$, it can be easily removed from the received signal, and as a result, it will not cause interference at receiver $2$.

The achievability strategy presented above describes a set of constraints on the rates, which is summerized as follows (loose upper-bounds have been eliminated):
\begin{equation}
\label{ach1}
\left\{ \begin{array}{ll}
R_1^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(1)}}{1 + {\sf INR_{21}} P_2^{(1)} } \right) \\
R_1^{(2)} &\leq \log \left( \frac{ {\sf SNR_1} P_1^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)} + {\sf SNR_1} P_1^{(1)} } \right) \\
R_1^{(3)} &\leq \min \{ \log \left( 1 + \frac{ {\sf SNR_1} P_1^{(3)}}{1 + {\sf INR_{21}} P_2 + {\sf SNR_1} P_1^{(1:2)} } \right), C_{\sf FB} \} \\
R_1^{(4)} &\leq \log \left( 1 + \frac{ {\sf INR_{12}} P_1^{(4)}}{1 + {\sf INR_{12}} P_1^{(1:2)} + {\sf SNR_2} P_2^{(1)}} \right) \\
R_2^{(1)} &\leq \log \left( 1 + \frac{ {\sf SNR_2} P_2^{(1)}}{1 + {\sf INR_{12}} P_1^{(1:2)} } \right) \\
R_2^{(2)} &\leq \log \left( \frac{ {\sf INR_{21}} P_2^{(2)}}{1 + {\sf INR_{21}} P_2^{(1)} + {\sf SNR_1} P_1^{(1)} } \right) \\
R_2^{(3)} &\leq \log \left( 1 + \frac{ {\sf INR_{21}} P_2^{(3)}}{1 + {\sf INR_{21}} P_2^{(1:2)} + {\sf SNR_1} P_1^{(1:2)} } \right)
\end{array} \right.
\end{equation}

Note that $X_1^{(3,b)}$ is the repetition of $W_2^{(2,b-2)}$ and as a result, it should not be considered as part of $R_1$ when calculating the achievable sum-rate.

{\bf Achievability Strategy 2:}

In some cases there is no need to decode superposition of messages and as a reslut, the scheme becomes simpler in such cases. We show how achievability strategy 1 can be adjusted accordingly. The aforementioned condition happens for the case of strong interference regime, \emph{i.e.} ${\sf INR_{12}} \geq {\sf SNR_1}$ and ${\sf INR_{21}} \geq {\sf SNR_2}$. In this case we set $R_1^{(1)}, R_1^{(2)}$ and $R_2^{(1)}$ equal to zero. In other words, $W_1^{(1)}, W_1^{(2)}$ and $W_2^{(1)}$ are deterministic messages. As for the feedback strategy, receiver $1$ decodes $X_2^{(2)}$ (instead of the superposition of $X_1^{(2)}$ and $X_2^{(2)}$) and sends the lattice index of $W_2^{(2)}$ back to transmitter $1$ during the following block. Transmitter $1$ later encodes this message as $X_1^{(3)}$ and transmits it. The decoding works very similar to what we described above and we get the following set of constraints to guarantee small error probability at the decoders.
